Efficient Reinforcement Learning Through Trajectory Generation

A key barrier to using reinforcement learning (RL) in many real-world applications is the requirement of a large number of system interactions to learn a good control policy. Off-policy and Offline RL methods have been proposed to reduce the number of interactions with the physical environment by learning control policies from historical data. However, their performances suffer from the lack of exploration and the distributional shifts in trajectories once controllers are updated. Moreover, most RL methods require that all states are directly observed, which is difficult to be attained in many settings. To overcome these challenges, we propose a trajectory generation algorithm, which adaptively generates new trajectories as if the system is being operated and explored under the updated control policies. Motivated by the fundamental lemma for linear systems, assuming sufficient excitation, we generate trajectories from linear combinations of historical trajectories. For linear feedback control, we prove that the algorithm generates trajectories with the exact distribution as if they are sampled from the real system using the updated control policy. In particular, the algorithm extends to systems where the states are not directly observed. Experiments show that the proposed method significantly reduces the number of sampled data needed for RL algorithms.

==> Trajectory Generation_longerv2/Preliminaries.tex <==

\subsection{Notations}


Throughout this manuscript, vectors are denoted in lower case bold and matrices are denoted in upper case bold, unless otherwise specified. Vectors of all ones and zeros are denoted by $\mathbbold{1}_n, \mathbbold{0}_n \in \real^n$, respectively. The identity matrix  is denoted by $\bm{I}_n\in\real^{n\times n}$. 
% \bz{none of the matrices or vectors are bold though}
% We use $\mathbb{N}, \mathbb{R}, \mathbb{R}_{\geq 0}$ and $\mathbb{R}_{>0}$ to denote the set of natural, real, nonnegative and positive real numbers, respectively. 
% For $A \in \mathbb{R}^{m \times n},[A]_i$ and $[A]_{i j}$ represent its $i$-th row and $(i, j)$-th element, respectively. 
We use $\mathcal{N}(\bm{A})$ to denote the null space of matrix $\bm{A}$. Given $n$ matrices $\bm{M}_i, i=1,\cdots,n$, we denote $[\bm{M}_1;\cdots;\bm{M}_n]:=[\bm{M}_1^\top \cdots \bm{M}_n^\top]^\top$.
% A continuous function $\alpha: \mathbb{R} \rightarrow \mathbb{R}$ is of (extended) class- $\mathcal{K}$ if it is strictly increasing and $\alpha(0)=0$. 



Given a discrete-time signal   $\bm{z}(t)\in \mathbb{R}^d$ for $t=0,1,\cdots$, we 
% adopt the notation
% in~\citep{de2019formulas} 
use $\bm{z}_{[k, k+T]}\in\real^{Td}$  to denote the vector form of the sequence $\{\bm{z}(k), \ldots, \bm{z}(k+T)\}$,
% for $k \in \mathbb{Z}, T \in \mathbb{N}$, 
and the Hankel matrix $\bm{Z}_{i, t, N}\in\real^{td\times N}$ as
% associated to the signal $\bm{z}$ as follows
\vspace{-0.1cm}
$$
\bm{Z}_{[k, k+T]}=\left[\begin{array}{c}
\bm{z}(k) \\
\vdots \\
\bm{z}(k+T)
\end{array}\right],
\bm{Z}_{i, t, N}=\left[\begin{array}{cccc}
\bm{z}(i) & \bm{z}(i+1) & \cdots & \bm{z}(i+N-1) \\
\bm{z}(i+1) & \bm{z}(i+2) & \cdots & \bm{z}(i+N) \\
\vdots & \vdots & \ddots & \vdots \\
\bm{z}(i+t-1) & \bm{z}(i+t) & \cdots & \bm{z}(i+t+N-2)
\end{array}\right],
$$
where $k,i$ and are integers, and $t, N, T $ are natural numbers. The first subscript of $\bm{Z}_{i, t, N}$ denotes the time at which the first sample of the signal is taken, the second one the number of samples per each column, and the last one the number of signal samples per each row. 
% \lh{not necessary to cite it here because you use the same notation system}
% Sometimes, if $t=1$, noting that the matrix $\bm{z}_{i, t, N}$ has only one block row, we simply write
% $$
% \bm{z}_{i, N}=\left[\begin{array}{llll}
% \bm{z}(i) & \bm{z}(i+1) & \cdots & \bm{z}(i+N-1)
% \end{array}\right] .
% $$









\subsection{Problem formulation}\label{subsec: problem}
We consider a  discrete-time linear time-invariant system
\vspace{-0.1cm}
\begin{equation}\label{eq:sys_full}
\begin{aligned}
\bm{x}(k+1) &=\bm{A} \bm{x}(k)+\bm{B} \bm{u}(k) \\
\bm{y}(k) &=\bm{C} \bm{x}(k)
\end{aligned}
\end{equation}
with state $\bm{x} \in \mathbb{R}^n$, action $\bm{u} \in \mathbb{R}^m$, and output  $\bm{y} \in \mathbb{R}^q$ (sometimes called observations in RL literature).  If $\bm{C}$ is not of full (column) rank, we say that the states are not directly observed. Otherwise, we assume $\bm{C}=\bm{I}_n$ and the states are directly observed.  We assume that $\bm{A}$ and $\bm{B}$ are not known. The matrix $\bm{C}$ is also unknown if the state is not directly observed. We also make the standard assumption that $\left(\bm{A},\bm{B}\right)$ is stabilizable and $\left(\bm{A},\bm{C}\right)$ observable~\citep{hespanha2009linear}. 
% \vspace{-0.1cm}
% \begin{assumption}
%  $\left(\bm{A},\bm{B}\right)$ is stabilizable and $\left(\bm{A},\bm{C}\right)$ observable. 
% \end{assumption}
 





A trajectory is a sequence of observations and actions of length $T$, given by $\bm{\tau}=\{\bm{y}(0), \bm{u}(0), \cdots \\ ,  \bm{y}(T-1), \bm{u}(T-1)\}$. The control action $\bm{u}(k)$ most commonly comes from the control policy conditioned on the observation at time $k$, written as  $\bm{\pi}_{\bm{\theta}}\left(\bm{u}(k) \mid \bm{y}(k)\right)$ with $\bm{\theta}$ being the parameter for the control policy. Let $c\left(\bm{\tau}\right)$ be the cost defined over the trajectory $\bm{\tau}$.  The goal is to optimize the control paramater $\bm{\theta}$ to minimize the expected cost over  trajectories, written as:
\vspace{-0.1cm}
\begin{equation}\label{eq:Opt_obj}
J(\bm{\theta})=\mathbb{E}_{\bm{\tau} \sim p_{\bm{\pi}_{\bm{\theta}}}}c\left(\bm{\tau}\right) ,    
\end{equation}
where $p_{\bm{\pi}_{\bm{\theta}}}$ is the probability distribution of  trajectory  subject to the policy $\bm{\pi}_{\bm{\theta}}$.
% is given by
% \begin{equation}\label{eq:prob_traj0}
% p_{\bm{\pi}_{\bm{\theta}}}(\bm{\tau})=p\left(\bm{x}(0)\right) \prod_{k=0}^{K-1} p\left(\bm{y}(k) \mid \bm{x}(k)\right) \bm{\pi}_{\bm{\theta}}\left(\bm{u}(k) \mid \bm{y}(k)\right) p\left(\bm{x}(k+1) \mid \bm{x}(k), \bm{u}(k)\right) .    
% \end{equation}
The definition of $c\left(\bm{\tau}\right)$ varies for different problems. 
For linear control policy, quadratic costs are most commonly utilized to convert the optimization into classical linear quadratic problems~\citep{fazel2018global,zheng2021sample}. There are typically not closed-form solutions for~\eqref{eq:Opt_obj} for other cost functions, e.g., $c\left(\bm{\tau}\right)=\sum_{i=1}^n\max_{k=0,\cdots,K-1}|x_i(k)|$ for the frequency control problem in power systems~\citep{cui2022tps}. In this case, gradient-based methods can be utilized to update $\bm{\theta}$, but the lack of system parameters makes it difficult to compute the gradient $ \nabla_{\bm{\theta}} J(\bm{\theta})$.

% For example, $c\left(\bm{\tau}\right)=\sum_{k=0}^{K-1}\bm{x}(k)^\top Q\bm{x}(k)+\bm{u}(k)^\top R\bm{u}(k)$ for classical , $c\left(\bm{\tau}\right)=\sum_{i=1}^n\allowbreak\max_{k=0,\cdots,K-1}|x_i(k)|$ for the power system frequency control in~\citep{cui2022tps} and $c\left(\bm{\tau}\right)=\sum_{k=0}^{K-1}||\bm{x}(k)||_1+\gamma||\bm{u}(k)||_1$ for the battery control in. 

% \begin{subequations}\label{eq:Optimization}
% \begin{align}
% \min_{\bm{\bm{\theta}}} & \quad J(\bm{\theta}) \label{subeq:Optimization_obj}\\
% \mbox{s.t. } 
%  &\bm{x}(k+1)=A \bm{x}(k)+B \bm{u}(k)   \label{subeq:Optimization_V}\\
%  & \bm{u}(k) = \bm{\theta} \bm{x}(k)\\
% & \bm{u} \text{ is stabilizing}\label{subeq:Optimization_stability}
% \end{align}
% \end{subequations}

% The goal in a reinforcement learning problem is to learn a policy, which defines a distribution over actions conditioned on states, $\bm{\pi}_{\bm{\theta}}\left(\bm{u}(k) \mid \bm{x}(k)\right)$.   


\paragraph{Direct policy gradient methods.} 
Reinforcement learning (RL) is proposed to update $\bm{\theta}$ through gradient descent, where the gradient $ \nabla_{\bm{\theta}} J(\bm{\theta})$ is  approximated  from trajectories of the system under the control policy $\bm{\pi}_{\bm{\theta}}$. 
For example, the policy gradient methods in~\citep{Sutton2018RL} shows that the gradient $ \nabla_{\bm{\theta}} J(\bm{\theta})$  can be equivalently computed by
\vspace{-0.1cm}
\begin{equation}\label{eq: PG_grad}
    \nabla_{\bm{\theta}} J(\bm{\theta}) = \mathbb{E}_{\bm{\tau} \sim p_{\bm{\pi}_{\bm{\theta}}}(\bm{\tau})}\left[c(\bm{\tau})\sum_{k=0}^{K-1} \nabla_{\bm{\theta}} \log p_{\bm{\pi}_{\bm{\theta}}}\left(\bm{u}(k) \mid \bm{y}(k)\right)\right], 
\end{equation}
where $K$ is the length of the trajectory. The terms inside the expectation can be computed purely from observations and actions in the trajectory. 


If $\bm{C}=\bm{I}_n$ in~\eqref{eq:sys_full}, the states are directly measured and the control law is called state-feedback control. Otherwise, the control law is called output-feedback control. 
Note that if $\bm{C}$ is not full column rank, then $(\bm{y}(t),\bm{u}(t))$ cannot uniquely determine $\bm{y}(t+1)$. Namely, the system is not a Markov decision process with respect to $(\bm{y}(t),\bm{u}(t))$ and it is difficult to use generic RL algorithms based on the quality function $Q((\bm{y}(t),\bm{u}(t))$~\citep{jin2020sample}.
For illustration purpose, this paper focus on the policy gradient algorithm~\eqref{eq: PG_grad}, and we consider both state and output feedback control. 
% Thus,  $\bm{\theta}$ is update through  the gradient $ \nabla_{\bm{\theta}} J(\bm{\theta})$  approximated  from trajectories of the system under the control policy $\bm{\pi}_{\bm{\theta}}$.
% Most RL methods are built on the Markov Decision process where the  observation-action pair  $(\bm{y}(k),\bm{u}(k))$ at the time step $k$ can uniquely determine the observation at the next time step (i.e., $\bm{y}(k+1)$).



% On this basis,  a quality function $Q_{\bm{\theta}}((\bm{y}(t),\bm{u}(t))$ is typically learned to approximate the cost function $J(\bm{\theta})$. The control policy $\bm{\pi}_{\bm{\theta}}$ is optimized subsequently using the learned quality function $Q_{\bm{\theta}}((\bm{y}(t),\bm{u}(t))$.  However, if $\bm{C}$ is not full column rank, then $(\bm{y}(t),\bm{u}(t))$ cannot uniquely determine $\bm{y}(t+1)$. Namely, the system is not a Markov decision process with respect to $(\bm{y}(t),\bm{u}(t))$. Correspondingly, the RL algorithms based on the quality function $Q((\bm{y}(t),\bm{u}(t))$ cannot be directly used. 
% For illustration purpose, this paper focus on policy gradient algorithm~\eqref{eq: PG_grad}.




\vspace{-0.1cm}
\subsection{Approximate gradients with sampled trajectories} 
% Throughout this paper, we  consider the linear feedback control law $\bm{u}(k)=\bm{\theta} \bm{y}(k)$, with $\bm{\theta}$ being the trainable parameter.
When online interactions with the system are limited, computing the expectation in~\eqref{eq: PG_grad} is not trivial even when the states are directly observed.
In training, the expectation in~\eqref{eq: PG_grad} is approximated by the sample average over a large number of trajectories $\bm{\tau}$ collected from the system under the control policy $\bm{\pi}_{\bm{\theta}}$. Since the distribution $p_{\bm{\pi}_{\bm{\theta}}}(\bm{\tau})$ depends on the parameter $\bm{\theta}$, a new set of trajectories need to be collected after each iteration of updating $\bm{\theta}$. Thus, the number of samples increases with the batchsize (i.e., the number of trajectories in each episode) and the number of training episodes.
% However, sampling on the true system may be expensive and implementing the control policy that has not been trained well may be dangerous.  

We seek to update the control policy using  historical trajectories and thus do not need to interact with the system during  training.  Two challenges arise: \textit{(i) Distribution Shift.}  If the control policy changes, the distribution of 
the historical trajectories would be different from the true distribution $p_{\bm{\pi}_{\bm{\theta}}}(\bm{\tau})$, potentially resulting in large errors when computing~\eqref{eq: PG_grad}. 
\textit{(ii) Exploration.} Most RL methods need to add (sometimes large) perturbations on actions to encourage exploration, but training with a fixed set of historical trajectories may limit exploration. 
% the explore of potential search region with lower cost.
% The large perturbations of actions typically do not exist in the past trajectories, thus training with past trajectories limits the exploration of policies.


% This is the well-known challenge of distribution shift problem in offline RL.





\paragraph{End-to-End Trajectory Generation.} We propose to overcome the challenges of distribution shift and the lack of exploration through generating trajectories from historical data. In this paper, we focus on learning linear feedback control law $\bm{u}(k)=\bm{\theta} \bm{y}(k)$, with $\bm{\theta}\in\real^{m\times q}$ being the matrix of trainable parameters. For exploration, 
the action during training follows the control policy with perturbations $\bm{w}(k)$ as additive noise, written as
\vspace{-0.1cm}
\begin{equation}\label{eq:control_policy}
\bm{\pi}_{\bm{\theta}}\left(\bm{u}(k) \mid \bm{y}(k)\right):=\left\{\bm{u}(k)=\bm{\theta} \bm{y}(k)+\bm{w}(k), \bm{w}(k)\sim\mathcal{D}\right\},
\end{equation}
where $\mathcal{D}$ is the prescribed distribution for the perturbations. The variance of $\mathcal{D}$  is typically initialized to be large and then shrink with the training episode to achieve  exploration v.s. exploitation. 


We provide a simple end-to-end approach to generate input-output trajectories without system identification, allowing it to  extend to systems where the states are not directly observed (i.e., when $\bm{C}$ is not full column rank). The generated trajectories  are guaranteed to  have the same distribution as $p_{\bm{\pi}_{\bm{\theta}}}(\bm{\tau})$ 
% in~\eqref{eq:prob_traj0}
for all $\bm{\theta}$ and $\mathcal{D}$.  We first show the trajectory generation algorithm for state-feedback control in Section~\ref{sec:TrajGen_FullState}, then generalize the results to output-feedback control in Section~\ref{sec: TrajGen_PartialState}.


% Note that the distribution of trajectories is dependent on the parameter $\bm{\theta}$. 
% The key challenge is to make  the distribution of the generated trajectory the same as $p_{\bm{\pi}_{\bm{\theta}}}(\bm{\tau})$ subject to the latest policy $\bm{\pi}_{\bm{\theta}}$.
% % in~\eqref{eq:prob_traj0}. 
%  % Moreover, it is difficult to quantify how close the distribution of the generate trajectories from the true distribution.
% For linear control policy with perturbations for exploration, this paper proposes an  algorithm to generate trajectory totally offline but guarantee to  have the same distribution as $p_{\bm{\pi}_{\bm{\theta}}}(\bm{\tau})$ 
% % in~\eqref{eq:prob_traj0}
% for all $\bm{\theta}$. We consider the control law $\bm{u}(k)=\bm{\theta} \bm{y}(k)+\bm{w}(k)$, where $\bm{w}(k)\sim\mathcal{D}$ is the perturbation on actions subject to zero-mean distribution $\mathcal{D}$. In the next section, we first show the trajectory generation algorithm when the states in the system are fully observed, then generalize the results to cases when the states are partially observed.
% % \lh{(are partially observed, let's stick to the terminology you defined)}.  

  



% After canceling all the terms in equal to one, the probability of a trajectory $\bm{\tau}$ derived in~\eqref{eq:prob_traj} is 
% \begin{equation}
% \begin{split}
%   \bm{\pi}_{\bm{\theta}}(\bm{\tau})= p\left(\bm{x}(0)\right) \prod_{t=0}^{T-1} &p\left(\bm{u}(t)|\bm{x}(t)\right).
% \end{split}
% \end{equation}






% \subsection{Fundamental Lemma}

% In this section, we revisit the main result in [27] and state a few auxiliary results inspired by subspace identification [2], which will be useful throughout the article.

% For the sake of simplicity, throughout the article, we consider a controllable and observable discrete-time linear system
% $$
% \begin{aligned}
% \bm{x}(k+1) &=A \bm{x}(k)+B \bm{u}(k) \\
% \bm{y}(k) &=C \bm{x}(k)+D \bm{u}(k)
% \end{aligned}
% $$
% where $x \in \mathbb{R}^n, u \in \mathbb{R}^m$, and $y \in \mathbb{R}^p$.
% The system input-output response of over $[0, t-1]$ can be expressed as
% $$
% \left[\begin{array}{l}
% u_{[0, t-1]} \\
% y_{[0, t-1]}
% \end{array}\right]=\left[\begin{array}{cc}
% I_{t m} & \mathcal{O}_{t m \times n} \\
% \mathcal{T}_t & \mathcal{O}_t
% \end{array}\right]\left[\begin{array}{c}
% u_{[0, t-1]} \\
% x_0
% \end{array}\right]
% $$
% where $x_0$ is the system initial state, and where
% $$
% \begin{aligned}
% \mathcal{T}_t &:=\left[\begin{array}{ccccc}
% D & 0 & 0 & \cdots & 0 \\
% C B & D & 0 & \cdots & 0 \\
% C A B & C B & D & \cdots & 0 \\
% \vdots & \vdots & \vdots & \ddots & \vdots \\
% C A^{t-2} B & C A^{t-3} B & C A^{t-4} B & \cdots & D
% \end{array}\right] \\
% \mathcal{O}_t &:=\left[\begin{array}{c}
% C \\
% C A \\
% \vdots \\
% C A^{t-1}
% \end{array}\right]
% \end{aligned}
% $$
% are the Toeplitz and observability matrices of order $t$.
% Let now $u_{d,[0, T-1]}$ and $y_{d,[0, T-1]}$ be the input-output data of the system collected during an experiment, and let


% $$
% \left[\begin{array}{cccc}
% U_{0, t, T-t+1} \\
% Y_{0, t, T-t+1}
% \end{array}\right]:=\left[\begin{array}{cccc}
% u_d(0) & u_d(1) & \cdots & u_d(T-t) \\
% u_d(1) & u_d(2) & \cdots & u_d(T-t+1) \\
% \vdots & \vdots & \ddots & \vdots \\
% u_d(t-1) & u_d(t) & \cdots & u_d(T-1) \\
% \hline y_d(0) & y_d(1) & \cdots & y_d(T-t) \\
% y_d(1) & y_d(2) & \cdots & y_d(T-t+1) \\
% \vdots & \vdots & \ddots & \vdots \\
% y_d(t-1) & y_d(t) & \cdots & y_d(T-1)
% \end{array}\right]
% $$
% be the corresponding Hankel matrix. 

% Similarly to (2), we can write
% where
% $$
% X_{0, T-t+1}=\left[\begin{array}{llll}
% x_d(0) & x_d(1) & \ldots & x_d(T-t)
% \end{array}\right]
% $$
% and $x_d(i)$ are the state samples. For $u_d, y_d$, and $x_d$, we use the subscript $d$ so as to emphasize that these are the sample data collected from the system during some experiment.



==> Trajectory Generation_longerv2/TrajGen_FullState.tex <==
% In this section, we show the trajectory generation algorithm when all states are directly observed \lh{(are fully observed)}, namely $\bm{C}=\bm{I}_n$ and $\bm{y}(t)=\bm{x}(t)$. We will extend the results to the case when $\bm{C}\neq\bm{I}_n$ in the next section.
In this section, we show the conditions when the linear combination of historic trajectories spans all possible trajectories. On this basis, we derive the algorithm to generate trajectories corresponding to updated control policies with   perturbations on actions for explorations.
\subsection{Span of historic trajectories}



% represented as
% $$
% \begin{aligned}
% \mathcal{T}_{[0, T-1]} :=\left[\begin{array}{ccccc}
% \bm{B} & \mathbbold{0}_{n\times m}  & \mathbbold{0}_{n\times m} & \cdots & \mathbbold{0}_{n\times m} \\
% \bm{A} \bm{B} & \bm{B} & \mathbbold{0}_{n\times m} & \cdots & \mathbbold{0}_{n\times m} \\
% \vdots & \vdots & \vdots & \ddots & \vdots \\
% \bm{A}^{T-2} \bm{B} & \bm{A}^{T-3} \bm{B} & \bm{A}^{T-4} \bm{B} & \cdots & \mathbbold{0}_{n\times m}
% \end{array}\right] 
% \quad\mathcal{O}_{[0, T-1]} :=\left[\begin{array}{c}
% \bm{I}_{n} \\
% \bm{A} \\
% \vdots \\
% \bm{A}^{T-1}
% \end{array}\right].
% \end{aligned}
% $$




Let $\bm{u}_{d,[0, L-1]}$ and $\bm{x}_{d,[0, L-1]}$ be the a length-$L$ input and state from past trajectory, and let the corresponding Hankel matrix $\mathcal{H}\in\real^{(Tm+Tn)\times (L-T+1})$ defined as
\vspace{-0.1cm}
\begin{equation}\label{eq:Hankel_u_x}
    \begin{split}
    &\underbrace{ 
    \begin{bmatrix}
\bm{U}_{0, T, L-T+1}  \\
\bm{X}_{0, T, L-T+1}     
    \end{bmatrix}
}_{\mathcal{H}}\quad
:=
\left[\begin{matrix}
\bm{u}_d(0) & \bm{u}_d(1) & \cdots & \bm{u}_d(L-T) \\
% \bm{u}_d(1) & \bm{u}_d(2) & \cdots & \bm{u}_d(L-T+1) \\
\vdots & \vdots & \ddots & \vdots \\
\bm{u}_d(T-1) & \bm{u}_d(T) & \cdots & \bm{u}_d(L-1) \\
\hline \bm{x}_d(0) & \bm{x}_d(1) & \cdots & \bm{x}_d(L-T) \\
% \bm{x}_d(1) & \bm{x}_d(2) & \cdots & \bm{x}_d(L-T+1) \\
\vdots & \vdots & \ddots & \vdots \\
\bm{x}_d(T-1) & \bm{x}_d(T) & \cdots & \bm{x}_d(L-1)
\end{matrix}\right].    
    \end{split}
\end{equation}

By the state-space version of  Fundamental Lemma~\citep{de2019formulas} shown below, any linear combination of the columns of the Hankel matrix is a length-$T$ input-state trajectory of~\eqref{eq:sys_full}. The proof is provided in~\citep{de2019formulas} and we supplement it in Appendix~\ref{app: fundemental}  for completeness.
 
% \LH{use command ``bmatrix'' $\begin{bmatrix} a \\ b \end{bmatrix}$ would save you some space.}



\vspace{-0.1cm}
\begin{lemma}[ Fundamental Lemma]\label{lem:fundemental}
%  Consider system (1). Then, the following holds.
% 1) If $u_{d,[0, T-1]}$ is persistently exciting of order $n+t$, 
If $\text{rank}\left[\begin{smallmatrix}
\bm{U}_{0, T, L-T+1} \\
\bm{X}_{0, L-T+1}
\end{smallmatrix}\right]=n+Tm$,
then any length-$T$ input/state trajectory of system~\eqref{eq:sys_full} can be expressed as
$\left[\begin{smallmatrix}
\bm{u}_{[0, T-1]} \\
\bm{x}_{[0, T-1]}
\end{smallmatrix}\right]=\left[\frac{\bm{U}_{0, T, L-T+1}}{\bm{X}_{0, T, L-T+1}}\right] \bm{g}$,
where $\bm{g}\in \mathbb{R}^{L-T+1}$.

% Moreover, any linear combination of the columns of the Hankel matrix, that is
% $$
% \left[\begin{array}{c}
% \bm{U}_{0, T, L-T+1} \\
% \hline \bm{X}_{0, T, L-T+1}
% \end{array}\right] \bm{g}
% $$
% is a length-$T$ input/state trajectory of~\eqref{eq:sys_full}.
\end{lemma}

For the rank condition in Lemma~\ref{lem:fundemental} to hold, the minimum requirement on the length of the collected trajectory is $L-T+1=n+Tm$, namely, $L=(m+1)T-1+n$. 
When the rank condition holds, linear combination of the columns of the Hankel matrix is also a length-$T$ trajectory of the system. Thus, we generate a trajectory of length $T$ using
\vspace{-0.1cm}
\begin{equation}\label{eq:Hankel_g0}
\begin{bmatrix}
\Tilde{\bm{u}}(0);
\cdots;
\Tilde{\bm{u}}(T-1);
\Tilde{\bm{x}}(0);
\cdots;
\Tilde{\bm{x}}(T-1)
\end{bmatrix}
=   
   \underbrace{ 
    \begin{bmatrix}
\bm{U}_{0, T, L-T+1}  \\
\bm{X}_{0, T, L-T+1}     
    \end{bmatrix}
}_{\mathcal{H}}\bm{g}.
\end{equation}

% \begin{equation}\label{eq:Hankel_g0}
%  \left[\begin{array}{c}
% \Tilde{\bm{u}}(0) \\
% \vdots\\
% \Tilde{\bm{u}}(T-1)\\
% \Tilde{\bm{x}}(0)\\
% \vdots\\
% \Tilde{\bm{x}}(T-1)
% \end{array}\right]=   
%   \underbrace{ \left[\begin{array}{cccc}
% \bm{U}_{0, T, L-T+1}  \\
% \bm{X}_{0, T, L-T+1} 
% \end{array}\right]}_{\mathcal{H}}\bm{g}
% \end{equation}

For convenience, we adopt the notation $\mathcal{H}_u=\bm{U}_{0, T, L-T+1} $, $\mathcal{H}_x=\bm{X}_{0, T, L-T+1} $ in the following sections. To represent the rows of blocks starting from the time $k=0,\cdots,T-1$, we denote
\vspace{-0.1cm}
\begin{equation}\label{eq:H_u_k}
\mathcal{H}_x^k :=
[
\bm{x}_d(k) \; \bm{x}_d(k+1)\,  \cdots\,  \bm{x}_d(L-T+k)
],\,
\mathcal{H}_u^k :=
[
\bm{u}_d(k) \; \bm{u}_d(k+1) \, \cdots \, \bm{u}_d(L-T+k)
].  
\end{equation}

% \begin{equation*}
% \mathcal{H}_x^k :=
% \begin{bmatrix}
% \bm{x}_d(k) & \bm{x}_d(k+1) & \cdots & \bm{x}_d(L-T+k)
% \end{bmatrix}
% \mathcal{H}_u^k :=
% \begin{bmatrix}
% \bm{u}_d(k) & \bm{u}_d(k+1) & \cdots & \bm{u}_d(L-T+k)
% \end{bmatrix}.  
% \end{equation*}

% \begin{equation}\label{eq:H_u_k}
% \mathcal{H}_u^k :=
% \begin{bmatrix}
% \bm{u}_d(k) & \bm{u}_d(k+1) & \cdots & \bm{u}_d(L-T+k)
% \end{bmatrix}.    
% \end{equation}




\subsection{Trajectory generation}

For generic RL algorithms, a trajectory is sampled from the system that starts from an initial state $\bm{x}(0)$ and subsequently implements the control policy  $\bm{u}(k)=\bm{\theta} \bm{x}(k)+\bm{w}(k), \bm{w}(k)\sim\mathcal{D}$  for $k=0,\cdots,T-1$. Given $\bm{\theta}$, the probability density function of a trajectory is
\vspace{-0.1cm}
\begin{equation}\label{eq:pdf}
\begin{split}
   p_{\pi_{\bm{\theta}}}(\bm{\tau})= p\left(\bm{x}(0)\right) \prod_{k=0}^{T-1} &p\left(\bm{\theta} \bm{x}(k)+\bm{w}(k)|\bm{x}(k)\right) p\left(\bm{x}(k+1) \mid \bm{x}(k), \bm{\theta} \bm{x}(k)+\bm{w}(k)\right),
\end{split}
\end{equation}
which is uniquely determined by $\bm{x}(0)$ and the sequence of perturbations $\bm{w}(0), \bm{w}(1),\cdots, \bm{w}(T-1)$. 


In the following, we generate trajectories for each updated $\bm{\theta}$ as if  they  truly come from the system starting from $\bm{x}(0)$ under perturbations on actions given by  $\bm{w}(0),\cdots, \bm{w}(T-1)$. 
 Importantly, we use fixed historic trajectories $\left\{\bm{u}_d, \bm{y}_d\right\}$ where the Hankel matrix $\mathcal{H}$ in~\eqref{eq:Hankel_u_x} satisfies $\text{rank}(\mathcal{H})=n+Tm$, and $\bm{u}_d$ can come from controllers different from the control policy in~\eqref{eq:control_policy}.
 
 
 The key is to use $\bm{x}(0)$ and $(\bm{w}(0),\allowbreak\cdots, \bm{w}(T-1))$ as extra constraints to find the $\bm{g}$ in~\eqref{eq:Hankel_g0} that generates the trajectory which follows the same distribution as~\eqref{eq:pdf}. 
From the control policy $\bm{u}(k)=\bm{\theta} \bm{x}(k)+\bm{w}(k)$, the trajectory subject to the perturbations  $\bm{w}(0), \bm{w}(1),\cdots, \bm{w}(T-1)$  should satisfy
\vspace{-0.1cm}
\begin{equation}\label{eq: costrains_w}
\begin{split}
 \left[\begin{array}{c}
\Tilde{\bm{u}}(0) \\
\vdots\\
\Tilde{\bm{u}}(T-1)\\
\end{array}\right]= 
\underbrace{\begin{bmatrix}
\bm{\theta}&  &  &  \\
 % &  \bm{\theta}&  &  \\
 &  &  \ddots&  \\
 &  &  & \bm{\theta} \\
\end{bmatrix}}_{\bm{I}_{T}\bigotimes\bm{\theta}}
 \left[\begin{array}{c}
\Tilde{\bm{x}}(0)\\
\vdots\\
\Tilde{\bm{x}}(T-1)
\end{array}\right] 
+\left[\begin{array}{c}
\bm{w}(0) \\
\vdots\\
\bm{w}(T-1)\\
\end{array}\right].    
\end{split}
\end{equation}

% \begin{equation}
%  \left[\begin{array}{c}
% \bm{u}(0) \\
% \vdots\\
% \bm{u}(T-1)\\
% \end{array}\right]= 
% \underbrace{\begin{bmatrix}
% \bm{\theta}&  &  &  \\
%  &  \bm{\theta}&  &  \\
%  &  &  \ddots&  \\
%  &  &  & \bm{\theta} \\
% \end{bmatrix}}_{\bm{I}_{T}\bigotimes\bm{\theta}}
%  \left[\begin{array}{c}
% \bm{x}(0)\\
% \vdots\\
% \bm{x}(T-1)
% \end{array}\right] 
% +\left[\begin{array}{c}
% \bm{w}(0) \\
% \vdots\\
% \bm{w}(T-1)\\
% \end{array}\right].
% \end{equation}

% Hence,the generated trajectory should also satisfy the system dynamics, which leads to
% \begin{equation}\label{eq: costrains_w}
% \begin{split}
% &\left[\begin{array}{c}
% \mathcal{H}_u
% \end{array}\right]\bm{g}\quad=\left(\bm{I}_{T}\otimes\bm{\theta}\right)
% \left[\begin{array}{cccc}
% \mathcal{H}_x
% \end{array}\right]\bm{g}
% +\left[\begin{array}{c}
% \bm{w}(0) \\
% \vdots\\
% \bm{w}(T-1)\\
% \end{array}\right].    
% \end{split}
% \end{equation}

Note that the generated initial state is given by $\Tilde{\bm{x}}(0)=\left[\begin{array}{cccc}
\mathcal{H}_x^0
\end{array}\right]\bm{g}$. Combining with~\eqref{eq: costrains_w} gives

% \begin{equation}
% \left[\begin{array}{cccc}
% \mathcal{H}_x^0
% \end{array}\right]:=\left[\begin{array}{cccc}
%  \bm{x}_d(0) & \bm{x}_d(1) & \cdots & \bm{x}_d(L-T) \\
% \end{array}\right],    
% \end{equation}




% Let
% \begin{equation}
%     R_{\bm{\theta}}:=\left[\begin{array}{cccc}
% \bm{U}_{0, T, L-T+1} 
% \end{array}\right]- \begin{bmatrix}
% \bm{\theta}&  &  &  \\
%  &  \bm{\theta}&  &  \\
%  &  &  \ddots&  \\
%  &  &  & \bm{\theta} \\
% \end{bmatrix}  
% \left[\begin{array}{cccc}
% \bm{X}_{0, T, L-T+1} 
% \end{array}\right]
% \end{equation}
\vspace{-0.1cm}

\begin{equation}\label{eq:traj_g0}
\underbrace{\begin{bmatrix}
\mathcal{H}_u-\left(\bm{I}_{T}\otimes\bm{\theta}\right) \mathcal{H}_x\\
\mathcal{H}_x^0
\end{bmatrix}}_{\bm{G}_{\bm{\theta}}}
\bm{g}=
\begin{bmatrix}
\bm{w}(0) \\
\vdots\\
\bm{w}(T-1)\\
\bm{x}(0)
\end{bmatrix}.
\end{equation}




Note that the matrix $\bm{G}_{\bm{\theta}}\in\real^{(Tm+n) \times (L-T+1)}$ is not a square matrix and its rank is determined by the length of historic trajectory $L$. When the trajectory is sufficiently long and  $\text{rank}(\mathcal{H})=n+Tm$, we have $L-T+1>Tm+n$ and thus there might be multiple $\bm{g} $ where~\eqref{eq:traj_g0} holds.
% Since all solution of~\eqref{eq:traj_g0} generates the unique trajectory, 
We use the  minimum-norm solution of~\eqref{eq:traj_g0} given by 
% \lh{(not sure if it is a good idea to mention noise in data, which also motivates the minimum-norm solution. I guess the reviewers will anyway ask you about how to deal with noisy data, but it is also okay to just let them ask.)}
\vspace{-0.1cm}
\begin{equation}\label{eq: g_star0}
    \bm{g}^*=\bm{G}_{\bm{\theta}}^\top\left(\bm{G}_{\bm{\theta}} \bm{G}_{\bm{\theta}}^\top\right)^{-1}\left[\begin{array}{c}
\bm{w}(0);
\cdots;
\bm{w}(T-1);
\bm{x}(0)
\end{array}\right].
\end{equation}


% \begin{equation}\label{eq: g_star0}
%     g^*=\bm{G}_{\bm{\theta}}^\top\left(\bm{G}_{\bm{\theta}} \bm{G}_{\bm{\theta}}^\top\right)^{-1}\left[\begin{array}{c}
% \bm{w}(0) \\
% \vdots\\
% \bm{w}(T-1)\\
% \bm{x}(0)
% \end{array}\right].
% \end{equation}




In the next Theorem, we prove  the existence and uniqueness of the trajectory generated by~\eqref{eq:traj_g0}. The goal is to show that given $\left(\bm{w}(0),\cdots ,\bm{w}(T-1), \bm{x}(0)\right)$, any $\bm{g} $  that satisfies~\eqref{eq:traj_g0}  will generate the same trajectory using $\mathcal{H}\bm{g}$. So it is suffice to choose the closed-form solution in~\eqref{eq: g_star0}. 


\vspace{-0.1cm}
\begin{theorem}\label{thm: unque_trajectory0}
If $\text{rank}(\mathcal{H})=n+Tm$, there exists at least one solution $\bm{g}$ such that~\eqref{eq:traj_g0} holds. 
Given $\left(\bm{w}(0),\cdots ,\bm{w}(T-1), \bm{x}(0)\right)$ and any $\bm{g} $  that solves~\eqref{eq:traj_g0},  $\mathcal{H}\bm{g}^*$ generates the same unique trajectory under the control policy~\eqref{eq:control_policy} parameterized by $\bm{\theta}$.
% For any solution $g^*$ of~\eqref{eq:traj_g0}, the generated trajectory given by 
% $[\Tilde{\bm{u}}(0);
%         \cdots;
%         \Tilde{\bm{u}}(T-1);
%         \Tilde{\bm{x}}(0);
%         \cdots;
%         \Tilde{\bm{x}}(T-1)]
%         =\mathcal{H}\bm{g}^*$ 
% % $\Big[
% %         \Tilde{\bm{u}}(0)^\top 
% %         \cdots
% %         \Tilde{\bm{u}}(T-1)^\top
% %         \Tilde{\bm{x}}(0)^\top 
% %         \cdots
% %         \Tilde{\bm{x}}(T-1)^\top
% %         \Big]^\top=\mathcal{H}\bm{g}^*$ 
%         is the unique trajectory starting from $\bm{x}(0)$ under perturbations on actions given by  $\bm{w}(0),\cdots, \bm{w}(T-1)$.
\end{theorem}


Theorem~\ref{thm: unque_trajectory0} shows that $\mathcal{H}\bm{g}^*$  generates the unique trajectory that starts from an initial state $\bm{x}(0)$ and subsequently implements the control policy  $\bm{u}(k)=\bm{\theta} \bm{x}(k)+\bm{w}(k), \bm{w}(k)\sim\mathcal{D}$. Hence, if we fix $\bm{\theta}$ in~\eqref{eq: g_star0} and sample $(\bm{x}(0), \bm{w}(0), \bm{w}(1),\cdots, \bm{w}(T-1))$, then $\mathcal{H}\bm{g}^*$  will generate a batch of  trajectories following the distribution~\eqref{eq:pdf} corresponding to the parameter $\bm{\theta}$. After the update of $\bm{\theta}$ in each episode of training, we generate a new batch of trajectories by updating $\bm{G}_{\bm{\theta}}$ in~\eqref{eq:traj_g0} and sampling new $(\bm{x}(0), \bm{w}(0), \bm{w}(1),\cdots, \bm{w}(T-1))$. Thus, the generated trajectories adaptively follow the shifted distribution after updating $\bm{\theta}$. Importantly, it overcomes the negative perception in the field that there is no possibility to improve explorations beyond past trajectories~\citep{levine2020offline}. By sampling the noises $\bm{w}(k)\sim\mathcal{D}$, explorations can also be achieved through the generated trajectories. Hence, new trajectories are adaptively generated as if the system were being operated and explored under the updated control policies.


To prove Theorem~\ref{thm: unque_trajectory0}, we first show that the null space of $\bm{G}_{\bm{\theta}}$ is exactly the same as  that of the Hankel matrix $\mathcal{H}$. Then,  $\text{rank}(\mathcal{H})=n+Tm$ yields $\text{rank}(\bm{G}_{\bm{\theta}})=n+Tm$. The full row rank of $\bm{G}_{\bm{\theta}}$ implies that there exist at least one $\bm{g}$ where~\eqref{eq:traj_g0} holds. The uniqueness of trajectory generated by $\bm{g}$  follows from the fact that $\bm{G}_{\bm{\theta}}$ and $\mathcal{H}$ have the same null space. Details of the proof is given below.

% \begin{lemma}\label{lem:null_full}
% The null space $\mathcal{N}(\bm{G}_{\bm{\theta}})$ is  the same as $\mathcal{N}(\mathcal{H})$. Moreover, if $\text{rank}(\mathcal{H})=n+Tm$, then the matrix $\bm{G}_{\bm{\theta}}\in\real^{(Tm+n) \times (L-T+1)}$ is full row rank. Namely, $\text{rank}(\bm{G}_{\bm{\theta}})=n+Tm$. 
% \end{lemma}
\begin{proof}
We first prove that the null space $\mathcal{N}(\bm{G}_{\bm{\theta}})$ is  the same as $\mathcal{N}(\mathcal{H})$ from \textit{(i)}  and \textit{(ii)} :


\textit{(i)} For all $\bm{q}\in \mathcal{N}(\mathcal{H})$,  we have $[\mathcal{H}_x]\bm{q} =\mathbbold{0}_{Tn}$ and $[\mathcal{H}_u]\bm{q} =\mathbbold{0}_{Tm}$. Plugging in  $\bm{G}_{\bm{\theta}}$ in~\eqref{eq:traj_g0} yields  $\bm{G}_{\bm{\theta}}\bm{q} = \mathbbold{0}_{Tm+n} $. Namely, $\bm{q}\in\mathcal{N}(\bm{G}_{\bm{\theta}})$.


\textit{(ii)} For all  $\bm{v}\in \mathcal{N}(\bm{G}_{\bm{\theta}})$,  $\bm{G}_{\bm{\theta}}\bm{v}=\mathbbold{0}_{Tm+n}$ yields $\mathcal{H}_x^0\bm{v} =\mathbbold{0}_{n}$ 
 and 
 $\mathcal{H}_u^k \bm{v}=\hat{\bm{\theta}}\mathcal{H}_x^k \bm{v} \text{ for  } k=0,\cdots,T-1$. Thus, $\mathcal{H}_u^0 \bm{v}=\hat{\bm{\theta}}\mathcal{H}_x^0 \bm{v}=\mathbbold{0}_{m}$. From $\bm{x}(k+1) =\bm{A} \bm{x}(k)+\bm{B} \bm{u}(k)$, we have $\mathcal{H}_x^{k+1}=A \mathcal{H}_x^{k}+B \mathcal{H}_u^{k}.$ From $ \mathcal{H}_x^{0}=\mathbbold{0}_{n}$ and $ \mathcal{H}_u^{0}=\mathbbold{0}_{m}$, we
apply $\mathcal{H}_x^{k+1}=A \mathcal{H}_x^{k}+B \mathcal{H}_u^{k}$ and $\mathcal{H}_u^k \bm{v}=\hat{\bm{\theta}}\mathcal{H}_x^k \bm{v}$ alternately. This induces
$\mathcal{H}_x^k \bm{v} =\mathbbold{0}_{n}$ and $\mathcal{H}_u^k \bm{v} =\mathbbold{0}_{m}$ for $ k=0,\cdots,T-1$. Hence, $\mathcal{H}\bm{v} = \mathbbold{0}_{Tm+Tn} $. 
% Namely, $\bm{v}\in\mathcal{N}(\mathcal{H})$. 
% From \textit{(i)}  and \textit{(ii)} , $\mathcal{N}(\bm{G}_{\bm{\theta}})$ is  the same as $\mathcal{N}(\mathcal{H})$.
% \begin{equation}
% \left[\begin{array}{c}
% \mathcal{H}_u-\left(\bm{I}_{T}\otimes\bm{\theta}\right) \mathcal{H}_x\\
% \mathcal{H}_x^0
% \end{array}\right]\bm{v}=\mathbbold{0}_{Tm+n}
% \end{equation}
% This gives 
% \begin{equation}\label{eq:fullC_null}
% \begin{split}
% &\mathcal{H}_x^0\bm{v} =\mathbbold{0}_{n} 
% \quad and \quad 
%  \mathcal{H}_u^k \bm{v}=\hat{\bm{\theta}}\mathcal{H}_x^k \bm{v} \text{ for  } k=0,\cdots,T-1
% \end{split}    
% \end{equation} 


% When $C$ is full-rank square matrix, we have  $y(k+1)=Cx(k+1)=C(A x(k)+B u(k))=CA C^{-1}y(k)+CB u(k)$. Hence,


% \begin{equation}~\label{eq:induction_x_u}
%     \mathcal{H}_x^{k+1}=A \mathcal{H}_x^{k}+B \mathcal{H}_u^{k}.
% \end{equation}


% Plugging~\eqref{eq:fullC_null} in~\eqref{eq:induction_x_u} induces
% $\mathcal{H}_x^k \bm{v} =\mathbbold{0}_{n}$ and $\mathcal{H}_u^k \bm{v} =\mathbbold{0}_{m}$ for $ k=0,\cdots,T-1$. Hence, $\mathcal{H}\bm{v} = \mathbbold{0}_{Tm+Tn} $. Namely, $\bm{v}\in\mathcal{N}(\mathcal{H})$.

Next, we prove the existence of the solution in~\eqref{eq:traj_g0}. Note that $\mathcal{H}\in\real^{(Tm+Tn) \times (L-T+1)}$. If $\text{rank}(\mathcal{H})=n+Tm$, then  $\text{rank}(\mathcal{N}(\mathcal{H}))=(L-T+1)-(n+Tm)$.  
Since $\mathcal{N}(\bm{G}_{\bm{\theta}})$ is  the same as $\mathcal{N}(\mathcal{H})$, then $\text{rank}(\mathcal{N}(\bm{G}_{\bm{\theta}}))=(L-T+1)-(n+Tm)$.  It follows directly that $\text{rank}(\bm{G}_{\bm{\theta}})=(L-T+1)-\text{rank}(\mathcal{N}(\bm{G}_{\bm{\theta}}))=n+Tm$.  Note that the number of rows of  $\bm{G}_{\bm{\theta}}$ is $n+Tm$, then the full row-rank of $\text{rank}(\bm{G}_{\bm{\theta}})$ shows that there exists at least one solution such that~\eqref{eq:traj_g0} holds.

Lastly, we show the uniqueness of the generated trajectory. Suppose there exists $\bm{g}_1$ and $\bm{g}_2$, which are both solutions of~\eqref{eq:traj_g0} and $\mathcal{H}\bm{g}_1\neq \mathcal{H}\bm{g}_2$. Since $\bm{g}_1$ and $\bm{g}_2$ are both solution of~\eqref{eq:traj_g0}, then $\bm{G}_{\bm{\theta}}\bm{g}_1=\bm{G}_{\bm{\theta}}\bm{g}_1$ and thus $\left(\bm{g}_1-\bm{g}_2\right)\in\mathcal{N}(\bm{G}_{\bm{\theta}})$.
On the other hand, $\mathcal{H}\bm{g}_1\neq \mathcal{H}\bm{g}_2$ yields $\mathcal{H}\left(\bm{g}_1-\bm{g}_2\right)\neq 0$ and thus $\left(\bm{g}_1-\bm{g}_2\right)\notin\mathcal{N}(\mathcal{H})$. This contradicts that $\mathcal{N}(\bm{G}_{\bm{\theta}})$ is  the same as $\mathcal{N}(\mathcal{H})$. Hence, $\mathcal{H}\bm{g}_1= \mathcal{H}\bm{g}_2$, namely, the generated trajectories are identical.
% Therefore, $\mathcal{H}\bm{g}^*$ generates the unique trajectory for any solution $g^*$ of~\eqref{eq:traj_g0}.
\end{proof}


% We are now ready to prove Theorem~\ref{thm: unque_trajectory0}.

% \begin{proof}
% By Lemma~\ref{lem:null_full}, $\text{rank}(\bm{G}_{\bm{\theta}})=n+Tm$ if $\text{rank}(\mathcal{H})=n+Tm$ .  Note that the number of rows of  $\bm{G}_{\bm{\theta}}$ is $n+Tm$, then $\text{rank}(\bm{G}_{\bm{\theta}})=n+Tm$ is full row-rank and therefore there exists at least one solution such that~\eqref{eq:traj_g0} holds.

% Suppose there exists $\bm{g}_1$ and $\bm{g}_2$ are both solution of~\eqref{eq:traj_g0} and $\mathcal{H}\bm{g}_1\neq \mathcal{H}\bm{g}_2$. Since $\bm{g}_1$ and $\bm{g}_2$ are both solution of~\eqref{eq:traj_g0}, then $\bm{G}_{\bm{\theta}}\bm{g}_1=\bm{G}_{\bm{\theta}}\bm{g}_1$ and thus $\left(\bm{g}_1-\bm{g}_2\right)\in\mathcal{N}(\bm{G}_{\bm{\theta}})$.
% On the other hand, $\mathcal{H}\bm{g}_1\neq \mathcal{H}\bm{g}_2$ yields $\mathcal{H}\left(\bm{g}_1-\bm{g}_2\right)\neq 0$ and thus $\left(\bm{g}_1-\bm{g}_2\right)\notin\mathcal{N}(\mathcal{H})$. This contradicts that $\mathcal{N}(\bm{G}_{\bm{\theta}})$ is  the same as $\mathcal{N}(\mathcal{H})$ proved in Lemma~\ref{lem:null_full}. Therefore, $\mathcal{H}\bm{g}^*$ generates the unique trajectory for any solution $g^*$ of~\eqref{eq:traj_g0}.
% \end{proof}





% From~\eqref{eq:Hankel_u_x(k)ransition}, the null space $\mathcal{N}(\mathcal{H})$ of the Hankel matrix  is $(L-T+1)-(n+Tm)$.
% If $x(t)$ is fully observable( or the length of $x(t)$ is the same as $x(t)$), then  the rank of null space $\mathcal{N}(\bm{G}_{\bm{\theta}})$ is also $(L-T+1)-(n+Tm)$. 


 

% \wc{I feel that we may not need to involve the case when historic trajectory is not enough. It increases lots of hyper-parameters that is not easy to elaborate clearly.}
%  During the period of data collection, the length of historic trajectory may not be long enough and thus  $\text{rank}(\bm{G}_{\bm{\theta}})<n+Tm$. In this case, we do not have to wait until the rank condition holds.  We generate trajectory by minimizing the reconstruction error $\min_g ||\bm{G}_{\bm{\theta}} g-[\bm{w}(0),\cdots,\bm{w}(T-1),\bm{x}(0)]^\top||_2^2$, which yields the closed-form solution
%  \begin{equation}
%     g=\left(\bm{G}_{\bm{\theta}}^\top \bm{G}_{\bm{\theta}} \right)^{-1}\bm{G}_{\bm{\theta}}^\top\left[\begin{array}{c}
% \bm{w}(0) \\
% \vdots\\
% \bm{w}(T-1)\\
% \bm{x}(0)
% \end{array}\right]
% \end{equation}
\vspace{-0.1cm}
\subsection{Algorithm}

By Theorem~\ref{thm: unque_trajectory0}, using historical data, given $\bm{x}(0)$ and perturbations on actions  $\bm{w}(0),\cdots, \bm{w}(T-1)$, 
a trajectory can be generated as if it comes from sampling the system with the current control policy.
The details of the algorithm is illustrated in Algorithm~\ref{alg: TrajGenFull}. 
We also use REINFORCE policy gradient~\citep{Sutton2018RL} in Appendix~\ref{app: PG_state_feedback} as an example to show how to use the trajectory generation algorithm in RL methods.
% We also use REINFORCE policy gradient~\citep{Sutton2018RL} in Algorithm~\ref{alg: PG} as an example to show how to integrate the trajectory generation algorithm in RL methods to train the controllers. 
The key benefit of Algorithm~\ref{alg: TrajGenFull}
% the trajectory generation algorithm 
is that it is adaptive to the updates of parameter $\bm{\theta}$ and  $\bm{w}(t)$ for exploration. In particular, $\bm{w}(t)$ can be sampled from any distribution $\mathcal{D}$, making it versatile for different applications.

\begin{algorithm}[h]
 \caption{Trajectory generation for state-feedback control }
 \label{alg: TrajGenFull}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Require: }}
 \renewcommand{\algorithmicensure}{\textbf{Data collection:}}
%  \REQUIRE  The length $T$ of trajectory to be generated, the dimension of state $n$, the dimension of action $m$
 \ENSURE Collect historic measurement of the system and stack each $T$-length input-output trajectory  as Hankel matrix $\mathcal{H}$ shown in~\eqref{eq:Hankel_u_x} until  $\text{rank}(\mathcal{H})=n+Tm$ \\
  \renewcommand{\algorithmicensure}{\textbf{Data generation:}}
 \ENSURE 
 \textit{Input} :Hankel matrix $\mathcal{H}$, weights $\bm{\theta}$ and the distribution $\mathcal{D}$ for the control policy,  the batchsize $Q$ (number of the generated  trajectories), the distribution $\mathcal{S}_x $ of the initial states\footnotemark \\
     \SetKwFunction{FMain}{TrajectoryGen}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$\mathcal{H},\bm{\theta},\mathcal{D},Q, \mathcal{S}_x  $}}{
          Plug in $\bm{\theta}$ to compute $\bm{G}_{\bm{\theta}}=\begin{bmatrix}
\mathcal{H}_u-\left(\bm{I}_{T}\otimes\bm{\theta}\right) \mathcal{H}_x;
\mathcal{H}_x^0
\end{bmatrix}$

        \For{$i = 1$ to $Q$}
        {Sample $\bm{x}_i(0)$ from $\mathcal{S}_x  $. Sample $\left\{\bm{w}_i(0),\cdots,\bm{w}_i(T-1)\right\}$ from  $\mathcal{D}$.\\
        Compute the  coefficient $\bm{g}_i^*=\bm{G}_{\bm{\theta}}^\top\left(\bm{G}_{\bm{\theta}} \bm{G}_{\bm{\theta}}^\top\right)^{-1}\left[
        \bm{w}_i(0);
        \cdots;
        \bm{w}_i(T-1);
        \bm{x}_i(0)
        \right]$.
        \\
        Generate the $i$-th trajectory    $\bm{\tau}_i:=\left[
        \Tilde{\bm{u}}_i(0);
        \cdots;
        \Tilde{\bm{u}}_i(T-1);
        \Tilde{\bm{x}}_i(0);
        \cdots;
        \Tilde{\bm{x}}_i(T-1);
        \right]=\mathcal{H}\bm{g}_i^*$.

        }
        \textbf{return} $ \left[\bm{\tau}_1,\cdots,\bm{\tau}_Q \right]$ 
        }
    % \textbf{End Function}
 \end{algorithmic} 
 \end{algorithm}
\footnotetext{The set of historic initial states in past trajectories can be used to estimate $\mathcal{S}_x $.}









==> Trajectory Generation_longerv2/Trajectory_Generation.tex <==

\subsection{Span of historic trajectories}


Expanding the system transition dynamics gives the input-state response  over $[0, T-1]$ as
$$
\left[\begin{array}{l}
\bm{u}_{[0, T-1]} \\
\bm{x}_{[0, T-1]}
\end{array}\right]=\left[\begin{array}{cc}
\bm{I}_{T m} & \mathbbold{0}_{T m \times n} \\
\mathcal{T}_{[0,T-1]} & \mathcal{O}_{[0,T-1]}
\end{array}\right]\left[\begin{array}{c}
\bm{u}_{[0, T-1]} \\
\bm{x}(0)
\end{array}\right]
$$
where $\bm{x}(0)$ is the system initial state, and
$$
\begin{aligned}
\mathcal{T}_{[0, T-1]} :=\left[\begin{array}{ccccc}
\bm{B} & \mathbbold{0}_{n\times m}  & \mathbbold{0}_{n\times m} & \cdots & \mathbbold{0}_{n\times m} \\
\bm{A} \bm{B} & \bm{B} & \mathbbold{0}_{n\times m} & \cdots & \mathbbold{0}_{n\times m} \\
\vdots & \vdots & \vdots & \ddots & \vdots \\
\bm{A}^{T-2} \bm{B} & \bm{A}^{T-3} \bm{B} & \bm{A}^{T-4} \bm{B} & \cdots & \mathbbold{0}_{n\times m}
\end{array}\right] 
\mathcal{O}_{[0, T-1]} :=\left[\begin{array}{c}
\bm{I}_{n} \\
\bm{A} \\
\vdots \\
\bm{A}^{T-1}
\end{array}\right]
\end{aligned}
$$
are the Toeplitz and observability matrices of order $T$.



Let now $\bm{u}_{d,[0, L-1]}$ and $\bm{x}_{d,[0, L-1]}$ be the  $L$-length input-output data  collected during an experiment, and let

\begin{equation}\label{eq:Hankel_u_x}
    \begin{split}
    &\left[\begin{array}{cccc}
\bm{U}_{0, T, L-T+1} \\
\bm{X}_{0, T, L-T+1}
\end{array}\right]\quad:=\left[\begin{array}{cccc}
\bm{u}_d(0) & \bm{u}_d(1) & \cdots & \bm{u}_d(L-T) \\
\bm{u}_d(1) & \bm{u}_d(2) & \cdots & \bm{u}_d(L-T+1) \\
\vdots & \vdots & \ddots & \vdots \\
\bm{u}_d(T-1) & \bm{u}_d(T) & \cdots & \bm{u}_d(L-1) \\
\hline \bm{x}_d(0) & \bm{x}_d(1) & \cdots & \bm{x}_d(L-T) \\
\bm{x}_d(1) & \bm{x}_d(2) & \cdots & \bm{x}_d(L-T+1) \\
\vdots & \vdots & \ddots & \vdots \\
\bm{x}_d(T-1) & \bm{x}_d(T) & \cdots & \bm{x}_d(L-1)
\end{array}\right]    
    \end{split}
\end{equation}

be the corresponding Hankel matrix $\mathcal{H}$. 

Let 
$$
\bm{X}_{0, L-T+1}:=\left[\begin{array}{llll}
\bm{x}_d(0) & \bm{x}_d(1) & \ldots & \bm{x}_d(L-T)
\end{array}\right].
$$

Then we have

\begin{equation}\label{eq:Hankel_u_\bm{x}(k)ransition}
\begin{bmatrix}
\bm{U}_{0, T, L-T+1} \\
\bm{X}_{0, T, L-T+1}
\end{bmatrix}
=\begin{bmatrix}
I_{T m} & \mathbbold{0}_{T m \times n} \\
\mathcal{T}_{[0,T-1]} & \mathcal{O}_{[0,T-1]}
\end{bmatrix}
\begin{bmatrix}
\bm{U}_{0, T, L-T+1}  \\
X_{0, L-T+1}
\end{bmatrix}   
\end{equation}

% \LH{use command ``bmatrix'' $\begin{bmatrix} a \\ b \end{bmatrix}$ would save you some space.}




Follow this expression, the fundamental Lemma shows that  any linear combination of the columns of the Hankel matrix is a T -long input/output trajectory of~\eqref{eq:sys_full}.

\begin{lemma}[Fundamental Lemma]\label{lem:fundemental}
%  Consider system (1). Then, the following holds.
% 1) If $u_{d,[0, T-1]}$ is persistently exciting of order $n+t$, 
If $\text{rank}\left[\begin{array}{cccc}
\bm{U}_{0, T, L-T+1}  \\
X_{0, L-T+1}
\end{array}\right]=n+Tm$,
then any $T$-long input/output trajectory of system~\eqref{eq:sys_full} can be expressed as
$$
\left[\begin{array}{l}
\bm{u}_{[0, T-1]} \\
\bm{x}_{[0, T-1]}
\end{array}\right]=\left[\frac{\bm{U}_{0, T, L-T+1} }{\bm{X}_{0, T, L-T+1} }\right] g
$$
where $g \in \mathbb{R}^{L-T+1}$.

Moreover, any linear combination of the columns of the Hankel matrix, that is
$$
\left[\begin{array}{c}
\bm{U}_{0, T, L-T+1}  \\
\hline \bm{X}_{0, T, L-T+1}
\end{array}\right] g
$$
is a $T$-long input/output trajectory of~\eqref{eq:sys_full}.
\end{lemma}

To make the rank condition in Lemma~\ref{lem:fundemental} hold,  the minimum requirement on the length of the collected data is $L-T+1=n+Tm$, namely, $L=(m+1)T-1+n$. 
When the rank condition holds, linear combination of the columns of the Hankel matrix is also a $T$-length trajectory of the system. We generate a trajectory of length $T$ using
\begin{equation}\label{eq:Hankel_g0}
 \left[\begin{array}{c}
\Tilde{\bm{u}}(0) \\
\vdots\\
\Tilde{\bm{u}}(T-1)\\
\Tilde{\bm{x}}(0)\\
\vdots\\
\Tilde{\bm{x}}(T-1)
\end{array}\right]=   
   \underbrace{ \left[\begin{array}{cccc}
\bm{U}_{0, T, L-T+1}   \\
\bm{X}_{0, T, L-T+1}  
\end{array}\right]}_{\mathcal{H}}g
\end{equation}

For convenience, we adopt the notation $\mathcal{H}_u=\bm{U}_{0, T, L-T+1}  $, $\mathcal{H}_x=\bm{X}_{0, T, L-T+1}  $ in the following sections. To represent the rows of blocks starting from the time $k=0,\cdots,T-1$, we denote

\begin{equation}
\mathcal{H}_x^k :=\left[\begin{array}{cccc}
\bm{x}_d(k) & \bm{x}_d(k+1) & \cdots & \bm{x}_d(L-T+k) \\
\end{array}\right]    
\end{equation}
\begin{equation}
\mathcal{H}_u^k :=\left[\begin{array}{cccc}
\bm{u}_d(k) & \bm{u}_d(k+1) & \cdots & \bm{u}_d(L-T+k) \\
\end{array}\right].    
\end{equation}




\subsection{Trajectory generation}

For generic policy gradient algorithm, a trajectory is collected from the system that start from a initial state $\bm{x}(0)$, subject to the control law  $\bm{u}(k)=\bm{\theta} \bm{x}(k)+\bm{w}(k)$ for $k=0,\cdots,T-1$. The probability density function of a trajectory is given by 
\begin{equation}\label{eq:pdf}
\begin{split}
   p_{\pi_\theta}(\tau)= p\left(\bm{x}(0)\right) \prod_{k=0}^{T-1} &p\left(\bm{w}(k)\right) p\left(\bm{x}(k+1) \mid \bm{x}(k), u(k)\right),
\end{split}
\end{equation}
which is uniquely determined by $\bm{x}(0)$ and the sequence of perturbations $\bm{w}(0), \bm{w}(1),\cdots, \bm{w}(T-1)$. 


In the following, we show the algorithm to generate the trajectory  subject to $\big\{\bm{x}(0),\bm{w}(0),\cdots, \allowbreak\bm{w}(T-1)\big\}$ from the Hankel matrix instead of truly implemented on the system. 


The key is to use $\left\{\bm{x}(0),\bm{w}(0),\cdots, \bm{w}(T-1)\right\}$ as extra constraint to find the $g$ in~\eqref{eq:Hankel_g0} that generate the same trajectory as if it is sampled from the system.


The trajectory subject to the noise vector  $\bm{w}(0), \bm{w}(1),\cdots, \bm{w}(T)$  satisfy
\begin{equation}
 \left[\begin{array}{c}
\Tilde{\bm{u}}(0) \\
\vdots\\
\Tilde{\bm{u}}(T)\\
\end{array}\right]= 
\underbrace{\begin{bmatrix}
\theta&  &  &  \\
 &  \theta&  &  \\
 &  &  \ddots&  \\
 &  &  & \theta \\
\end{bmatrix}}_{I_{T}\bigotimes\theta}
 \left[\begin{array}{c}
\Tilde{\bm{x}}(0)\\
\vdots\\
\Tilde{\bm{x}}(T)
\end{array}\right] 
+\left[\begin{array}{c}
\bm{w}(0) \\
\vdots\\
\bm{w}(T)\\
\end{array}\right]
\end{equation}

This indicates
\begin{equation}
\begin{split}
&\left[\begin{array}{c}
\mathcal{H}_u
\end{array}\right]g\quad= \begin{bmatrix}
\theta&  &  &  \\
 &  \theta&  &  \\
 &  &  \ddots&  \\
 &  &  & \theta \\
\end{bmatrix}  
\left[\begin{array}{cccc}
\mathcal{H}_x
\end{array}\right]g
+\left[\begin{array}{c}
\bm{w}(0) \\
\vdots\\
\bm{w}(T)\\
\end{array}\right]    
\end{split}
\end{equation}

Note that
\begin{equation}
\left[\begin{array}{cccc}
\mathcal{H}_x^0
\end{array}\right]:=\left[\begin{array}{cccc}
 \bm{x}_d(0) & \bm{x}_d(1) & \cdots & \bm{x}_d(L-T) \\
\end{array}\right],    
\end{equation}


the generated initial state is given by
\begin{equation}
    \Tilde{\bm{x}}(0)=\left[\begin{array}{cccc}
\mathcal{H}_x^0
\end{array}\right]g.
\end{equation}

% Let
% \begin{equation}
%     R_\theta:=\left[\begin{array}{cccc}
% \bm{U}_{0, T, L-T+1}  
% \end{array}\right]- \begin{bmatrix}
% \theta&  &  &  \\
%  &  \theta&  &  \\
%  &  &  \ddots&  \\
%  &  &  & \theta \\
% \end{bmatrix}  
% \left[\begin{array}{cccc}
% \bm{X}_{0, T, L-T+1}  
% \end{array}\right]
% \end{equation}




The generated trajectory should satisfy

\begin{equation}\label{eq:traj_g0}
\underbrace{\begin{bmatrix}
\mathcal{H}_u-\left(I_{T}\otimes\theta\right) \mathcal{H}_x\\
\mathcal{H}_x^0
\end{bmatrix}}_{G_\theta}
g=
\begin{bmatrix}
\bm{w}(0) \\
\vdots\\
\bm{w}(T-1)\\
\bm{x}(0)
\end{bmatrix}.
\end{equation}


Note that the matrix $G_\theta\in\real^{(Tm+n) \times (L-T+1)}$ is not a square matrix and its rank is determined by the length of historic trajectory $L$. When there is sufficient length of trajectory such that $\text{rank}(\mathcal{H})=n+Tm$, we have $L-T+1>Tm+n$ and thus there might be multiple $g $ such that~\eqref{eq:traj_g0} holds. We show in the next Lemma that the Null space of $G_\theta$ is exactly the same as the Hankel matrix $\mathcal{H}$. Hence, any $g $ such that~\eqref{eq:traj_g0} holds will generate the unique trajectory subject to $\left\{\bm{x}(0),\bm{w}(0),\cdots, \bm{w}(T-1)\right\}$.


% \begin{equation}\label{eq:traj_g}
% \begin{bmatrix}
% \bm{U}_{0, T, L-T+1}  -\left(I_{T}\otimes\theta\right) \bm{X}_{0, T, L-T+1}  \\
% \mathcal{H}_x^0
% \end{bmatrix}
% g=
% \begin{bmatrix}
% \bm{w}(0) \\
% \vdots\\
% \bm{w}(T-1)\\
% \bm{x}(0)
% \end{bmatrix}
% \end{equation}


\begin{lemma}
The null space $\mathcal{N}(G_\theta)$ is  the same as $\mathcal{N}(\mathcal{H})$. Moreover, if $\text{rank}(\mathcal{H})=n+Tm$, then the matrix $G_\theta\in\real^{(Tm+n) \times (L-T+1)}$ is full row rank. Namely, $\text{rank}(G_\theta)=n+Tm$. 
\end{lemma}
\begin{proof}
For all $q\in \mathcal{N}(\mathcal{H})$,  we have $[\mathcal{H}_x] q =\mathbbold{0}_{Tn}$ and $[\bm{U}_{0, T, L-T+1} ] q =\mathbbold{0}_{Tm}$. Plugging in the expression of $G_{\theta}$ yields  $G_{\theta}q = \mathbbold{0}_{Tm+n} $. Namely, $q\in\mathcal{N}(G_{\theta})$.


For all  $v\in \mathcal{N}(G_\theta)$,  we have
\begin{equation}
\left[\begin{array}{c}
\mathcal{H}_u-\left(I_{T}\otimes\theta\right) \mathcal{H}_x\\
\mathcal{H}_x^0
\end{array}\right]v=\mathbbold{0}_{Tm+n}
\end{equation}
This gives 
\begin{equation}\label{eq:fullC_null}
\begin{split}
&\mathcal{H}_u^k v=\hat{\theta}\mathcal{H}_x^k v \text{ for  } k=0,\cdots,T-1\\
&\mathcal{H}_x^0v =\mathbbold{0}_{n}  
\end{split}    
\end{equation} 


% When $C$ is full-rank square matrix, we have  $y(k+1)=C\bm{x}(k+1)=C(A \bm{x}(k)+B u(k))=CA C^{-1}y(k)+CB u(k)$. Hence,
From $\bm{x}(k+1)=A \bm{x}(k)+B u(k)$, we have
\begin{equation}
    \mathcal{H}_x^{k+1}=A \mathcal{H}_x^{k}+B \mathcal{H}_u^{k}
\end{equation}


Pluging in~\eqref{eq:fullC_null} yields 
$\mathcal{H}_x^k v =\mathbbold{0}_{n}$ and $\mathcal{H}_u^k v =\mathbbold{0}_{m}$ for $ k=0,\cdots,T-1$. Hence, $\mathcal{H}v = \mathbbold{0}_{Tm+Tn} $. Namely, $v\in\mathcal{N}(\mathcal{H})$.


Note that $H\in\real^{(Tm+Tn) \times (L-T+1)}$. If $\text{rank}(\mathcal{H})=n+Tm$, then the rank of Null space is $\text{rank}(\mathcal{N}(\mathcal{H}))=(L-T+1)-(n+Tm)$.  
Since $\mathcal{N}(G_\theta)$ is  the same as $\mathcal{N}(\mathcal{H})$, then $\text{rank}(\mathcal{N}(G_\theta))=(L-T+1)-(n+Tm)$.  It follows directly that $\text{rank}(\mathcal{H})=(L-T+1)-\text{rank}(\mathcal{N}(G_\theta))=n+Tm$. 


 


% ************
% Split the first $m$ row of the Hankel matrix gives
% \begin{equation}
% G_\theta:=
% \left[\begin{array}{c}
% [\bm{U}_{0, T, L-T+1} ]_{0}-\hat{\theta}[\bm{X}_{0, T, L-T+1} ]_{0}\\
% \hline
% [\bm{U}_{0, T, L-T+1} ]_{1:T-1} -\left(I_{T-1}\otimes\theta\right)[\bm{X}_{0, T, L-T+1} ]_{1:T-1}\\
% \hline
% [\bm{X}_{0, T, L-T+1} ]_{0}
% \end{array}\right]
% \end{equation}
% If $\text{rank}(G_\theta)<n+Tm$, then there exists a nonzero vector $v\in\real^{Tm+n}$ such that $v^\top G_\theta=\mathbbold{0}_{L-T+1}$. We split the vector $v$ such that $v=(v_0, v_1,v_2) $, where $v_0=[v]_{0:m-1}$, $v_1=[v]_{m:Tm-1}$, $v_2=[v]_{Tm:Tm+n-1}$. Then
% \begin{equation}
% \begin{split}
% v^\top G_\theta=& v_0^\top \left([\bm{U}_{0, T, L-T+1} ]_{0}-\hat{\theta}[\bm{X}_{0, T, L-T+1} ]_{0}\right)+v_2^\top \left([\bm{X}_{0, T, L-T+1} ]_{0}\right)  \\
% &\quad+v_1^\top \left([\bm{U}_{0, T, L-T+1} ]_{1:T-1} -\left(I_{T-1}\otimes\theta\right)[\bm{X}_{0, T, L-T+1} ]_{1:T-1}\right)\\
% =& \left[\begin{array}{cc}
% v_0^\top&v_1^\top
% \end{array}\right]\bm{U}_{0, T, L-T+1} 
% +
% \left(-v_0^\top\hat{\theta}+v_2^\top\right)[\bm{X}_{0, T, L-T+1} ]_{0}\\
% &\quad-v_1^\top \left(I_{T-1}\otimes\theta\right)[\bm{X}_{0, T, L-T+1} ]_{1:T-1}
% \\
% =& \left[\begin{array}{ccc}
% v_0^\top&v_1^\top&-v_0^\top\hat{\theta}+v_2^\top
% \end{array}\right]
% \left[\begin{array}{c}
% \bm{U}_{0, T, L-T+1} \\
% \left [\bm{X}_{0, T, L-T+1} \right ]_{0}
% \end{array}\right]\\
% &\quad-v_1^\top \left(I_{T-1}\otimes\theta\right)M_y
% \left[\begin{array}{c}
% \bm{U}_{0, T, L-T+1} \\
% \left [\bm{X}_{0, T, L-T+1} \right ]_{0}
% \end{array}\right]
% \end{split}
% \end{equation}
\end{proof}


% From~\eqref{eq:Hankel_u_\bm{x}(k)ransition}, the null space $\mathcal{N}(\mathcal{H})$ of the Hankel matrix  is $(L-T+1)-(n+Tm)$.
% If $\bm{x}(t)$ is fully observable( or the length of $\bm{x}(t)$ is the same as $\bm{x}(t)$), then  the rank of null space $\mathcal{N}(G_\theta)$ is also $(L-T+1)-(n+Tm)$. 


If $\text{rank}(G_\theta)=n+Tm$, then there exist at least one solution such that~\eqref{eq:traj_g0} holds. We pick the  minimum-norm solution of~\eqref{eq:traj_g0} given by


\begin{equation}
    g=G_\theta^\top\left(G_\theta G_\theta^\top\right)^{-1}\left[\begin{array}{c}
\bm{w}(0) \\
\vdots\\
\bm{w}(T-1)\\
\bm{x}(0)
\end{array}\right].
\end{equation}

% \wc{I feel that we may not need to involve the case when historic trajectory is not enough. It increases lots of hyper-parameters that is not easy to elaborate clearly.}
%  During the period of data collection, the length of historic trajectory may not be long enough and thus  $\text{rank}(G_\theta)<n+Tm$. In this case, we do not have to wait until the rank condition holds.  We generate trajectory by minimizing the reconstruction error $\min_g ||G_\theta g-[\bm{w}(0),\cdots,\bm{w}(T-1),\bm{x}(0)]^\top||_2^2$, which yields the closed-form solution
%  \begin{equation}
%     g=\left(G_\theta^\top G_\theta \right)^{-1}G_\theta^\top\left[\begin{array}{c}
% \bm{w}(0) \\
% \vdots\\
% \bm{w}(T-1)\\
% \bm{x}(0)
% \end{array}\right]
% \end{equation}


The proposed trajectory generation algorithm is illustrated as follows

\begin{algorithm}
 \caption{Policy Gradient with trajectory generation when the state is observable }
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Require: }}
 \renewcommand{\algorithmicensure}{\textbf{Data collection:}}
 \REQUIRE  The length $T$ of trajectory to be generated, the dimension of state $n$, the dimension of action $m$, the learning rate $\alpha$
 \ENSURE Collect historic measurement of the system and stack each $T$-length input-output trajectory  as Hankel matrix $\mathcal{H}$ shown in~\eqref{eq:Hankel_u_x} until  $\text{rank}(\mathcal{H})=n+Tm$ \\
  \renewcommand{\algorithmicensure}{\textbf{Policy Gradient with Data generation:}}
 \ENSURE 
%  Generate a batch of $Q$ trajectories of the length $T$ subject to the control law $u(t)=\theta \bm{x}(t)+\bm{w}(t)$, $\bm{w}(t)\sim \mathcal{D}$.  \\
 \textit{Initialisation} :Initial weights $\theta$ for control network
 \FOR {$episode = 1$ to $I$}
 \STATE Plug in $\theta$ to compute $G_\theta=\begin{bmatrix}
\mathcal{H}_u-\left(I_{T}\otimes\theta\right) \mathcal{H}_x\\
\mathcal{H}_x^0
\end{bmatrix}$
 \FOR {$i = 1$ to $Q$}
 \STATE Uniformly sample $x^i(0)$ from historic measurement of the system. Sample $\left\{w^i(0),\cdots,w^i(T-1)\right\}$ from the distribution $\mathcal{D}$.
 \STATE Compute the  coefficient $g_i=G_\theta^\top\left(G_\theta G_\theta^\top\right)^{-1}\left[
w^i(0)^\top 
\cdots
w^i(T-1)^\top
x^i(0)^\top
\right]^\top$
\STATE Generate the $i$-th trajectory    $\tau_i:=\left[
\Tilde{\bm{u}}^i(0)^\top 
\cdots
\Tilde{\bm{u}}^i(T-1)^\top
\Tilde{\bm{x}}^i(0)^\top 
\cdots
\Tilde{\bm{x}}^i(T-1)^\top
\right]^\top=\mathcal{H}g_i$
 \ENDFOR
 \STATE Compute the gradient $ \nabla J(\theta) =  \frac{1}{Q}\sum_{i=1}^{Q} c(\tau_i)\sum_{t=1}^{T} \nabla_{\theta}\log\pi_{\theta} (\Tilde{\bm{u}}^i(t)|\Tilde{\bm{x}}^i(t)) $
  \STATE  Update weights in the neural network by gradient descent:
  $\theta \leftarrow \theta-\alpha \nabla J(\theta) $
  \ENDFOR
 \end{algorithmic} 
 \end{algorithm}





==> Trajectory Generation_longerv2/experiment.tex <==
We end the paper with case studies for the control of the batch reactor system in~\citep{de2019formulas} and the power distribution system in~\citep{cui2022decentralized}. Both state-feedback and output-feedback control are studied in these systems. Detailed simulation setting and results are provided in  Appendix~\ref{app:exp_reactor} and Appendix~\ref{app:exp_voltage}. 
Code is available at 
\url{https://github.com/Wenqi-Cui/Trajectory-Generation}. Major simulation results are summarized below. 
\paragraph{Experiment Setup.} 
 We use REINFORCE policy gradient algorithm~\citep{Sutton2018RL} to train a linear feedback controller, with the goal to minimize  the cost of trajectories with length $K$. 
Let $E$ be the number of episode in training and $Q$ be the batch size of trajectories collected for each episode, respectively. Standard policy gradient algorithms needs  $Q\times K \times E$ samples. 
 We compare the performance of the REINFORCE policy gradient algorithm using the generated trajectories (labeled as PG-TrajectoryGen) and the same algorithm using trajectories sampled by interacting with the system (labeled as PG-Sample-Q for the batchsize Q). For testing, we randomly sample 800 initial states and compare the cost on trajectories starting from these states. 
 
\paragraph{State-feedback control in a batch reactor system.}
We use the model of a batch reactor system in~\citep{de2019formulas} , where $\bm{x}(t)\in\real^4, \bm{u}(t)\in\real^2$. The time horizon is $K=30$. Since the state is observed, we setup $T=K=30$ and collect historic trajectory of length $L = (m + 1)T -1 + n=93$ such that $\text{rank}(\mathcal{H})=n+Tm$. With a sampling period of 0.1s, the data collection takes 9.3s. We generate trajectories using Algorithm~\ref{alg: TrajGenFull} with a batch size of 1200 in each  episode. 
% , we can generate any batch of trajectories without any new steps of sampled data from the real system. 
 Figure~\ref{fig:Loss_AB_full_main}(a) and Figure~\ref{fig:Loss_AB_full_main}(b) shows the training and the testing loss, respectively.
 PG-TrajectoryGen attains the same performance as  PG-Sample-1200, since Theorem~\ref{thm: unque_trajectory0} guarantees that we generate trajectories  as if it were truly sampled on the system. Moreover,  Figure~\ref{fig:Loss_AB_full_main}(a)-(c) shows that the loss attained by   PG-Sample-Q reduces with larger Q, but it comes at the expense of increased number of samples from the system. By contrast, the number of samples in PG-TrajectoryGen purely comes
from the fixed historic trajectory of the length $L=93$, which is much smaller than PG-Sample-10 that needs $10\times30\times400=120000$ online samples. 
% where the length of samples is 120000 (equals to $10\times30\times400$).





\vspace{-0.1cm}

\begin{figure}[H]
\centering
\subfigure[Training Loss]{\includegraphics[width=1.8in]{figure/Loss_ABfull.png}}
% \subfigure[Testing-FullObs]{\includegraphics[width=1.4in]{figure/Loss_ABfull_test.png}}
\subfigure[Testing Loss]{\includegraphics[width=1.8in]{figure/Loss_ABfull_batchVSLoss.png}}
\subfigure[Number of samples]{\includegraphics[width=1.8in]{figure/Loss_ABfull_BatchVSsample.png}}
\vspace*{-3mm}
\caption{Performance of learning state-feedback controllers in the batch reactor system. PG-TrajectoryGen achieves the same loss as PG-Sample-1200 with much less samples.}\label{fig:Loss_AB_full_main}
\end{figure}



\vspace{-0.8cm}
\paragraph{Output-feedback control in a power distribution network.}
We further conduct experiments on the voltage control problem in IEEE 33bus test feeder~\citep{baran1989network, cui2022decentralized}, where $\bm{x}(t)\in\real^{32}$. We assume only 20 buses are measured and controlled, so $\bm{y}(t),\bm{u}(t)\in\real^{20}$. The observability matrix $\mathcal{O}_{[0, T_0]}(\bm{A}, \bm{C})$ becomes full column rank when $T_0=3$. The time horizon of trajectory is $K=20$. According to the trajectory generation algorithm developed in Subsection~\ref{subsec: TrajGenPartial}, we setup $T=K+T_0-1=22$ and collect historic trajectory of length $L = (m + 1)T -1 + n=493$. With a sampling period of 1s, data collection takes 493s. Figure~\ref{fig:Loss_voltage_partial_main}(a)-(c) compares the training loss, testing loss and the number of samples, respectively.  PG-TrajectoryGen achieves the same training and testing loss as PG-Sample-1000 with much smaller number of samples.





\vspace{-0.1cm}
\begin{figure}[H]
\centering
\subfigure[Training Loss]{\includegraphics[width=1.8in]{figure/Loss_voltage_partial.png}}
% \subfigure[Testing-FullObs]{\includegraphics[width=1.4in]{figure/Loss_ABfull_test.png}}
\subfigure[Testing Loss]{\includegraphics[width=1.8in]{figure/Loss_voltagePartial_batchVSLoss.png}}
\subfigure[Number of samples]{\includegraphics[width=1.8in]{figure/Loss_voltagePartial_BatchVSsample.png}}
\vspace*{-3mm}
\caption{Performance of learning output-feedback controllers in power distribution network. PG-TrajectoryGen achieves the same loss as PG-Sample-1000 with much less samples.}\label{fig:Loss_voltage_partial_main}
\end{figure}

==> Trajectory Generation_longerv2/intro.tex <==
We study the control of networked physical systems, where a large number of individual subsystems are connected to each other and operate in tandem. Such networked systems are present in numerous applications, and understanding their behaviors has been an active line of research~\cite{arcak2016networks,coogan2014dissipativity,simpson2018equilibrium}.
Currently, much of the effort have focused on characterizing properties of the subsystems and their interconnections to certify system stability. At the same time, the performance of these systems, that is, their ability to achieve certain objectives, is also of critical importance. The existing approaches, however, do not offer a framework to optimize system performance. 

In this paper, we develop structured neural network-based controllers that not only guarantee stability, but also establishes a framework for performance optimization. In particular, we consider networked systems where the output of the subsystems need to reach an agreement at the steady state~\cite{burger2014duality,dorfler2014synchronization}. For example, vehicles in a platoon need to reach the same velocity~\cite{coogan2014dissipativity}  and generators in a power grid need to reach the same speed~\cite{cui2022tps}. This steady state should also be reached as quickly as possible, making transient performance of the system important. At the steady state, we want to select the control that achieves output agreement with the lowest possible cost.
% since there are often many set points at the individual systems that lead to the same output value at the steady state, we want to find one that also optimize the cost.
% the transient process before reaching the steady state should 

% We study the control  of safety-critical  networked systems, where  individual physical systems are interconnected to realize cooperative target, including output agreement and performance optimization~\cite{arcak2016networks, burger2014duality, cui2021reinforcement, coogan2014dissipativity}. Such networked system should be stable under control, meaning that the system need to settle down to an acceptable steady state after a disturbance happens~\cite{arcak2016networks, coogan2014dissipativity}. Transient process refers to the period before reaching the steady-state, and the goal of controller design for transient stage is to reach steady state quicker with lower control effort. In addition, we aim to regulate the points where the control actions settles down, such that the required output agreement is attained 
% with the minimum cost~\cite{burger2014duality, Zhao2015acc,jiang2022stable}.
% For example, power systems consist of synchronous generators that are interconnected by the transmission lines. These generators are required to reach the agreement of synchronous with the same speed (60 Hz in North America).  Since there are many ways to set generator power outputs  to achieve this, we would like the output of generators to settle down to the configuration where  the total generation cost is minimized~\cite{Zhao2015acc, jiang2022stable}. 



% Each node only observe the local information and sometimes can communicate with limited neighbours, thus  static local control law and distributed algorithms are required to realize optimization targets.  These controller should still guarantee  stability and output agreement. Moreover, we want to optimize the controllers to realize better performance, which typically include reducing smaller control effort and smaller state deviation from their targeted value.

For the system without real-time computation capability, linear Proportional-Integral (PI)  controllers are almost always used in practice to achieve the above goals~\cite{Zhao2015acc, andreasson2014distributed,  weitenberg2018exponential, golnaraghi2017automatic}. 
A proportional term provides instant feedback to improve the transient performance and an integral term drives the system outputs to the desired value at the steady state~\cite{Zhao2015acc, andreasson2014distributed}. 
% Importantly, linear PI controllers have provable stability guarantees for a large range of systems.
If communication is available, previous works~\cite{Zhao2015acc, andreasson2014distributed,  weitenberg2018exponential, golnaraghi2017automatic, SCHIFFER2017auto} also tailor the integral term to realize distributed optimal resource allocation under quadratic costs. A linear parameterization, however, fundamentally restricts the degrees of freedom of a controller and can lead to very suboptimal performances. 
  

% Learning-based approaches have been proposed to parameterize nonlinear controllers as neural networks, which are then trained to optimize performance~\cite{zhang2021multi, qu2020scalable, wang2021multi,chu2019multi}. However, providing provable guarantees on stability and steady-state optimality has been challenging. In particular, it is nontrivial to certify stability for \textit{all} the possible initial states in a compact set. Recent works showed that monotonic controllers provably stabilize the system~\cite{cui2022tps,shi2021stability}, but they rely on  tailor-made Lyapunov functions and are limited to specific applications.
% %~\cite{huang2019adaptive,chen2021reinforcement}

In the last decade, learning based approaches become popular for nonlinear controller optimization over a host of objective functions~\cite{zhang2021multi, qu2020scalable, wang2021multi,chu2019multi}. The nonlinear control law is normally represented through neural networks, which can then be optimized through learning algorithms.  Many empirical works show that learning based approaches improve the performance by  at least 10\%-50\%  compared with conventional linear approaches for problems on robotics \cite{he2020reinforcement}, traffic systems~\cite{yuan2022reinforcement}, power systems~\cite{wang2021multi, shi2021stability, cui2022tps, cui2021lyapunov}, etc. However, providing provable guarantees on stability and steady-state optimality has been challenging. 

In particular, it is nontrivial to certify stability for \textit{all} the possible initial states in a compact set.  Most works require a linear system model, and sometimes also linear controller, such as LQR problems and its variants~\cite{fazel2018global, lisafe}. Decentralized and distributed neural network-based controller design are proposed to reduce the dependency on communications and global state observations~\cite{li2021distributed, mukherjee2020distributed}. 
The stability for nonlinear system model is more difficult. Many works add soft penalty on the violation of stability conditions in the cost function, but it cannot guarantee stability for all the possible initial states~\cite{chang2019neural}. 
Our previous works in~\cite{furieri2022distributed, cui2022tps,shi2021stability} shows that stabilizing structure can be enforced in the design of neural networks, but  they rely on  tailor-made Lyapunov functions and are limited to specific applications.
%~\cite{huang2019adaptive,chen2021reinforcement}




Moreover, current learning-based approaches generally only optimize transient performance but neglect optimality at the steady-state. Even when training with long time horizons is computationally feasible, it is difficult to quantify how long is enough to cover the steady state. On the other hand, linear PI controllers can achieve stability and steady-state optimality for a large range of systems. This work addresses the following open question:
 \textit{Can learning be structured to guarantee stability and steady-state optimality for a generalized class of networked systems?}


Clearly, it is not possible to design a controller for everything and the answer depends on picking the right abstraction of the system. Passivity is a classical notion in control theory to characterize the inherent property of dynamical
systems by how their inputs and outputs correlate~\cite{arcak2016networks}. Many systems have been shown to be equilibrium-independent
passive (EIP)~\cite{burger2014duality,cui2022equilibrium,meissen2017passivity}, which characterize passivity referenced to an arbitrary equilibrium input/output pair. This abstraction allows us to design generalized controllers for networked systems without considering their detailed dynamics. 
% This provides benefits for  generalized controller design, where the network-level study is based on passivity properties as abstractions of their detailed dynamical models.

\textbf{Contributions.} This paper focuses on controller design for networked systems where the node dynamics are EIP. We propose a structured neural-PI controller that has provable guarantees on stability and achieves steady-state optimal resource allocation. The key structure we use are monotonically increasing functions, and they are parameterized by what we call \emph{monotone neural networks}. This way, transient performances are optimized by training neural networks, while stability and steady-state optimality are guaranteed by design. Experiments on traffic and power system control demonstrate that the proposed approach can reduce the transient cost by at least 30\% compared to the best linear controllers and ensure the optimal steady state cost.  Unstructured neural networks, on ther other hand, lead to unstable behaviors. We summarize contributions as follows.
\begin{enumerate}[noitemsep,nolistsep,leftmargin=*, label=\arabic*)]
    \item We construct a framework of neural network-based controller design that optimizes both transient and steady-state behavior of networked systems. We adopt a modular approach of stability analysis based on equilibrium-independent passivity, making the framework scalable to large systems and also robust to topology and parameter variations.
    \item For networked systems without communication, we propose a neural-PI control law that can be implemented fully decentralizedly with only local information. In Theorem~\ref{thm: output_level_stable}, we prove that the controller design guarantees asymptotic stability and output agreement at the target value. In Theorem~\ref{thm:stack_relu}, we explicitly characterize the structural conditions of monotone neural networks and prove their universal approximation capability of monotonic functions.
    %the controller design and engineer neural networks to satisfy them implicitly. 
    \item If a communication network is available, we propose a neural-PI control law where neighbouring nodes can exchange information of their marginal costs. In Theorem~\ref{thm:equilibrium_cost}, we prove that this design guarantees both stability criteria and steady-state optimal resource allocation for a range of functions that includes, but is not restricted to, quadratic cost functions. 
\end{enumerate}




    %  All of the controllers are structured with monotonic increasing functions,
% allowing us to engineer neural networks and thus achieve steady-state performance guarantee by design. This provide a tractable approach optimize transient performances by learning while.
    % For the networks with communication, we propose structured controller design such that the steady-state optimal resource allocation can also be guaranteed with zero tracking error. This is realized by local updates with limited information exchange with neighbours, which indicates that the setpoints directly settle down to the optimal resource allocation solution distributedly without centralized optimization.


==> Trajectory Generation_longerv2/model.tex <==


% For the systems where the states cannot be directly observed ( $\bm{C}\neq\bm{I}_n$), output feedback control is adopted. If $\bm{C}$ is a full column rank, then $\bm{x}(t)$ can be uniquely recovered from $\bm{y}(t)$ using the relation  $\bm{x}(t)=(\bm{C}^\top\bm{C})^{-1}\bm{C}^\top\bm{y}(k)$. Correspondingly, $\bm{y}(k+1)=\bm{C}(\bm{C}^\top\bm{C})^{-1}\bm{C}^\top\bm{y}(k)+\bm{C}\bm{B}\bm{u}(k)$. Then the algorithm in Section~\ref{sec:TrajGen_FullState} directly works by replacing $\bm{x}$ with $\bm{y}$.
% On the other hand, if $\bm{C}$ is not full column rank, then $\bm{y}(k+1)$ cannot be determined by $(\bm{y}(k),\bm{u}(k))$, namely,
% the system is not a Markov decision process with respect to $(\bm{y}(k),\bm{u}(k))$ at one time step. In the following part of this section, we focus on the case when $\bm{C}$ is not full column rank. We will show that the system is a Markov decision process by defining an extended state using input-output
%  trajectory. On this basis, the trajectory generation algorithm also works by defining on the extended state. 

% As discussed in Subsection~\ref{subsec: problem}, $\bm{y}(k+1)$ cannot be determined by $(\bm{y}(k),\bm{u}(k))$ if $\bm{C}$ is not full column rank for the output-feedback control. Thus, the algorithm derived in the previous section cannot be directly used by replacing $\bm{x}$ using  $\bm{y}$. 
In this section, we show how to obtain a Markov decision process by defining an extended state using input-output
 trajectory. 
 % Then the high-level idea of trajectory generation is identical to Section~\ref{sec:TrajGen_FullState}.
 The key difference to Section~\ref{sec:TrajGen_FullState} is that $\bm{G}_{\bm{\theta}}$ may not be full row rank even when the rank condition on the Hankel matrix holds. Thus, the coefficients for generated trajectories and associated proofs are more nuanced. 

\subsection{Extended states for constructing Markov decision process}

% We show that the system is a Markov decision process in terms of trajectory of observations.



Let $
\mathcal{O}_{[0, \ell]}(\bm{A}, \bm{C}):=\operatorname{col}\left(\bm{C}, \bm{C} \bm{A}, \ldots, \bm{C} \bm{A}^{\ell-1}\right)
$ be the extended observability matrix.
The lag of the system~\eqref{eq:sys_full} is defined by the smallest integer $\ell\in \mathbb{Z}_{\geq 0}$ such that the observability matrix $\mathcal{O}_{[0, \ell]}(\bm{A}, \bm{C})$ has rank $n$, i.e., the state can be reconstructed from $\ell$ measurements~\citep{huang2021robust}.

Let $T_0\geq\ell$ be the length of a trajectory. 
Define the extended states as
\vspace{-0.1cm}
\begin{equation}
\mathcal{X}(k-1) :=\left[\begin{array}{c}
\bm{y}(k-T_0);
\cdots ;
\bm{y}(k-1);
\bm{u}(k-T_0);
\cdots ;
\bm{u}(k-2)
\end{array}\right].        
\end{equation}

% \begin{equation}
% \mathcal{X}(k-1) :=\left[\begin{array}{c}
% \bm{y}(k-T_0)\\
% \vdots \\
% \bm{y}(k-1)\\
% \bm{u}(k-T_0)\\
% \vdots \\
% \bm{u}(k-2)\\
% \end{array}\right]        
% \end{equation}

Then extending the system transition from time step 0 to $T_0$ gives 
\vspace{-0.1cm}
\begin{equation}\label{eq:sys_extended}
\mathcal{X}(k)=\Tilde{\bm{A}}\mathcal{X}(k-1)+\Tilde{\bm{B}}\bm{u}(k-1)
\text{ for } k\geq T_0, k\in\mathbb{Z},    
\end{equation}
which is a Markov decision process in terms of the extended states. Detailed proof and the definition of system transition matrix $(\Tilde{\bm{A}},\Tilde{\bm{B}})$ is given in Appendix~\ref{app: transition_partial}.
For the output-feedback control law in~\eqref{eq:control_policy},
% $\bm{u}(k)=\bm{\theta} \bm{y}(k)+\bm{w}(k)$
we have  $ p\left(\bm{u}(k)|\mathcal{X}(k)\right)=p\left(\bm{u}(k)|\bm{y}(k)\right)   
$ and it is straightforward to show that policy gradient algorithm using~\eqref{eq: PG_grad} still works. The proof is given in Appendix~\ref{app:Policy Gradient}.


==> Trajectory_Generation.tex <==

\subsection{Span of historic trajectories}


Expanding the system transition dynamics gives the input-state response  over $[0, T-1]$ as
$$
\left[\begin{array}{l}
\bm{u}_{[0, T-1]} \\
\bm{x}_{[0, T-1]}
\end{array}\right]=\left[\begin{array}{cc}
\bm{I}_{T m} & \mathbbold{0}_{T m \times n} \\
\mathcal{T}_{[0,T-1]} & \mathcal{O}_{[0,T-1]}
\end{array}\right]\left[\begin{array}{c}
\bm{u}_{[0, T-1]} \\
\bm{x}(0)
\end{array}\right]
$$
where $\bm{x}(0)$ is the system initial state, and
$$
\begin{aligned}
\mathcal{T}_{[0, T-1]} :=\left[\begin{array}{ccccc}
\bm{B} & \mathbbold{0}_{n\times m}  & \mathbbold{0}_{n\times m} & \cdots & \mathbbold{0}_{n\times m} \\
\bm{A} \bm{B} & \bm{B} & \mathbbold{0}_{n\times m} & \cdots & \mathbbold{0}_{n\times m} \\
\vdots & \vdots & \vdots & \ddots & \vdots \\
\bm{A}^{T-2} \bm{B} & \bm{A}^{T-3} \bm{B} & \bm{A}^{T-4} \bm{B} & \cdots & \mathbbold{0}_{n\times m}
\end{array}\right] 
\mathcal{O}_{[0, T-1]} :=\left[\begin{array}{c}
\bm{I}_{n} \\
\bm{A} \\
\vdots \\
\bm{A}^{T-1}
\end{array}\right]
\end{aligned}
$$
are the Toeplitz and observability matrices of order $T$.



Let now $\bm{u}_{d,[0, L-1]}$ and $\bm{x}_{d,[0, L-1]}$ be the  $L$-length input-output data  collected during an experiment, and let

\begin{equation}\label{eq:Hankel_u_x}
    \begin{split}
    &\left[\begin{array}{cccc}
\bm{U}_{0, T, L-T+1} \\
\bm{X}_{0, T, L-T+1}
\end{array}\right]\quad:=\left[\begin{array}{cccc}
\bm{u}_d(0) & \bm{u}_d(1) & \cdots & \bm{u}_d(L-T) \\
\bm{u}_d(1) & \bm{u}_d(2) & \cdots & \bm{u}_d(L-T+1) \\
\vdots & \vdots & \ddots & \vdots \\
\bm{u}_d(T-1) & \bm{u}_d(T) & \cdots & \bm{u}_d(L-1) \\
\hline \bm{x}_d(0) & \bm{x}_d(1) & \cdots & \bm{x}_d(L-T) \\
\bm{x}_d(1) & \bm{x}_d(2) & \cdots & \bm{x}_d(L-T+1) \\
\vdots & \vdots & \ddots & \vdots \\
\bm{x}_d(T-1) & \bm{x}_d(T) & \cdots & \bm{x}_d(L-1)
\end{array}\right]    
    \end{split}
\end{equation}

be the corresponding Hankel matrix $\mathcal{H}$. 

Let 
$$
\bm{X}_{0, L-T+1}:=\left[\begin{array}{llll}
\bm{x}_d(0) & \bm{x}_d(1) & \ldots & \bm{x}_d(L-T)
\end{array}\right].
$$

Then we have

\begin{equation}\label{eq:Hankel_u_\bm{x}(k)ransition}
\begin{bmatrix}
\bm{U}_{0, T, L-T+1} \\
\bm{X}_{0, T, L-T+1}
\end{bmatrix}
=\begin{bmatrix}
I_{T m} & \mathbbold{0}_{T m \times n} \\
\mathcal{T}_{[0,T-1]} & \mathcal{O}_{[0,T-1]}
\end{bmatrix}
\begin{bmatrix}
\bm{U}_{0, T, L-T+1}  \\
X_{0, L-T+1}
\end{bmatrix}   
\end{equation}

% \LH{use command ``bmatrix'' $\begin{bmatrix} a \\ b \end{bmatrix}$ would save you some space.}




Follow this expression, the fundamental Lemma shows that  any linear combination of the columns of the Hankel matrix is a T -long input/output trajectory of~\eqref{eq:sys_full}.

\begin{lemma}[Fundamental Lemma]\label{lem:fundemental}
%  Consider system (1). Then, the following holds.
% 1) If $u_{d,[0, T-1]}$ is persistently exciting of order $n+t$, 
If $\text{rank}\left[\begin{array}{cccc}
\bm{U}_{0, T, L-T+1}  \\
X_{0, L-T+1}
\end{array}\right]=n+Tm$,
then any $T$-long input/output trajectory of system~\eqref{eq:sys_full} can be expressed as
$$
\left[\begin{array}{l}
\bm{u}_{[0, T-1]} \\
\bm{x}_{[0, T-1]}
\end{array}\right]=\left[\frac{\bm{U}_{0, T, L-T+1} }{\bm{X}_{0, T, L-T+1} }\right] g
$$
where $g \in \mathbb{R}^{L-T+1}$.

Moreover, any linear combination of the columns of the Hankel matrix, that is
$$
\left[\begin{array}{c}
\bm{U}_{0, T, L-T+1}  \\
\hline \bm{X}_{0, T, L-T+1}
\end{array}\right] g
$$
is a $T$-long input/output trajectory of~\eqref{eq:sys_full}.
\end{lemma}

To make the rank condition in Lemma~\ref{lem:fundemental} hold,  the minimum requirement on the length of the collected data is $L-T+1=n+Tm$, namely, $L=(m+1)T-1+n$. 
When the rank condition holds, linear combination of the columns of the Hankel matrix is also a $T$-length trajectory of the system. We generate a trajectory of length $T$ using
\begin{equation}\label{eq:Hankel_g0}
 \left[\begin{array}{c}
\Tilde{\bm{u}}(0) \\
\vdots\\
\Tilde{\bm{u}}(T-1)\\
\Tilde{\bm{x}}(0)\\
\vdots\\
\Tilde{\bm{x}}(T-1)
\end{array}\right]=   
   \underbrace{ \left[\begin{array}{cccc}
\bm{U}_{0, T, L-T+1}   \\
\bm{X}_{0, T, L-T+1}  
\end{array}\right]}_{\mathcal{H}}g
\end{equation}

For convenience, we adopt the notation $\mathcal{H}_u=\bm{U}_{0, T, L-T+1}  $, $\mathcal{H}_x=\bm{X}_{0, T, L-T+1}  $ in the following sections. To represent the rows of blocks starting from the time $k=0,\cdots,T-1$, we denote

\begin{equation}
\mathcal{H}_x^k :=\left[\begin{array}{cccc}
\bm{x}_d(k) & \bm{x}_d(k+1) & \cdots & \bm{x}_d(L-T+k) \\
\end{array}\right]    
\end{equation}
\begin{equation}
\mathcal{H}_u^k :=\left[\begin{array}{cccc}
\bm{u}_d(k) & \bm{u}_d(k+1) & \cdots & \bm{u}_d(L-T+k) \\
\end{array}\right].    
\end{equation}




\subsection{Trajectory generation}

For generic policy gradient algorithm, a trajectory is collected from the system that start from a initial state $\bm{x}(0)$, subject to the control law  $\bm{u}(k)=\bm{\theta} \bm{x}(k)+\bm{w}(k)$ for $k=0,\cdots,T-1$. The probability density function of a trajectory is given by 
\begin{equation}\label{eq:pdf}
\begin{split}
   p_{\pi_\theta}(\tau)= p\left(\bm{x}(0)\right) \prod_{k=0}^{T-1} &p\left(\bm{w}(k)\right) p\left(\bm{x}(k+1) \mid \bm{x}(k), u(k)\right),
\end{split}
\end{equation}
which is uniquely determined by $\bm{x}(0)$ and the sequence of perturbations $\bm{w}(0), \bm{w}(1),\cdots, \bm{w}(T-1)$. 


In the following, we show the algorithm to generate the trajectory  subject to $\big\{\bm{x}(0),\bm{w}(0),\cdots, \allowbreak\bm{w}(T-1)\big\}$ from the Hankel matrix instead of truly implemented on the system. 


The key is to use $\left\{\bm{x}(0),\bm{w}(0),\cdots, \bm{w}(T-1)\right\}$ as extra constraint to find the $g$ in~\eqref{eq:Hankel_g0} that generate the same trajectory as if it is sampled from the system.


The trajectory subject to the noise vector  $\bm{w}(0), \bm{w}(1),\cdots, \bm{w}(T)$  satisfy
\begin{equation}
 \left[\begin{array}{c}
\Tilde{\bm{u}}(0) \\
\vdots\\
\Tilde{\bm{u}}(T)\\
\end{array}\right]= 
\underbrace{\begin{bmatrix}
\theta&  &  &  \\
 &  \theta&  &  \\
 &  &  \ddots&  \\
 &  &  & \theta \\
\end{bmatrix}}_{I_{T}\bigotimes\theta}
 \left[\begin{array}{c}
\Tilde{\bm{x}}(0)\\
\vdots\\
\Tilde{\bm{x}}(T)
\end{array}\right] 
+\left[\begin{array}{c}
\bm{w}(0) \\
\vdots\\
\bm{w}(T)\\
\end{array}\right]
\end{equation}

This indicates
\begin{equation}
\begin{split}
&\left[\begin{array}{c}
\mathcal{H}_u
\end{array}\right]g\quad= \begin{bmatrix}
\theta&  &  &  \\
 &  \theta&  &  \\
 &  &  \ddots&  \\
 &  &  & \theta \\
\end{bmatrix}  
\left[\begin{array}{cccc}
\mathcal{H}_x
\end{array}\right]g
+\left[\begin{array}{c}
\bm{w}(0) \\
\vdots\\
\bm{w}(T)\\
\end{array}\right]    
\end{split}
\end{equation}

Note that
\begin{equation}
\left[\begin{array}{cccc}
\mathcal{H}_x^0
\end{array}\right]:=\left[\begin{array}{cccc}
 \bm{x}_d(0) & \bm{x}_d(1) & \cdots & \bm{x}_d(L-T) \\
\end{array}\right],    
\end{equation}


the generated initial state is given by
\begin{equation}
    \Tilde{\bm{x}}(0)=\left[\begin{array}{cccc}
\mathcal{H}_x^0
\end{array}\right]g.
\end{equation}

% Let
% \begin{equation}
%     R_\theta:=\left[\begin{array}{cccc}
% \bm{U}_{0, T, L-T+1}  
% \end{array}\right]- \begin{bmatrix}
% \theta&  &  &  \\
%  &  \theta&  &  \\
%  &  &  \ddots&  \\
%  &  &  & \theta \\
% \end{bmatrix}  
% \left[\begin{array}{cccc}
% \bm{X}_{0, T, L-T+1}  
% \end{array}\right]
% \end{equation}




The generated trajectory should satisfy

\begin{equation}\label{eq:traj_g0}
\underbrace{\begin{bmatrix}
\mathcal{H}_u-\left(I_{T}\otimes\theta\right) \mathcal{H}_x\\
\mathcal{H}_x^0
\end{bmatrix}}_{G_\theta}
g=
\begin{bmatrix}
\bm{w}(0) \\
\vdots\\
\bm{w}(T-1)\\
\bm{x}(0)
\end{bmatrix}.
\end{equation}


Note that the matrix $G_\theta\in\real^{(Tm+n) \times (L-T+1)}$ is not a square matrix and its rank is determined by the length of historic trajectory $L$. When there is sufficient length of trajectory such that $\text{rank}(\mathcal{H})=n+Tm$, we have $L-T+1>Tm+n$ and thus there might be multiple $g $ such that~\eqref{eq:traj_g0} holds. We show in the next Lemma that the Null space of $G_\theta$ is exactly the same as the Hankel matrix $\mathcal{H}$. Hence, any $g $ such that~\eqref{eq:traj_g0} holds will generate the unique trajectory subject to $\left\{\bm{x}(0),\bm{w}(0),\cdots, \bm{w}(T-1)\right\}$.


% \begin{equation}\label{eq:traj_g}
% \begin{bmatrix}
% \bm{U}_{0, T, L-T+1}  -\left(I_{T}\otimes\theta\right) \bm{X}_{0, T, L-T+1}  \\
% \mathcal{H}_x^0
% \end{bmatrix}
% g=
% \begin{bmatrix}
% \bm{w}(0) \\
% \vdots\\
% \bm{w}(T-1)\\
% \bm{x}(0)
% \end{bmatrix}
% \end{equation}


\begin{lemma}
The null space $\mathcal{N}(G_\theta)$ is  the same as $\mathcal{N}(\mathcal{H})$. Moreover, if $\text{rank}(\mathcal{H})=n+Tm$, then the matrix $G_\theta\in\real^{(Tm+n) \times (L-T+1)}$ is full row rank. Namely, $\text{rank}(G_\theta)=n+Tm$. 
\end{lemma}
\begin{proof}
For all $q\in \mathcal{N}(\mathcal{H})$,  we have $[\mathcal{H}_x] q =\mathbbold{0}_{Tn}$ and $[\bm{U}_{0, T, L-T+1} ] q =\mathbbold{0}_{Tm}$. Plugging in the expression of $G_{\theta}$ yields  $G_{\theta}q = \mathbbold{0}_{Tm+n} $. Namely, $q\in\mathcal{N}(G_{\theta})$.


For all  $v\in \mathcal{N}(G_\theta)$,  we have
\begin{equation}
\left[\begin{array}{c}
\mathcal{H}_u-\left(I_{T}\otimes\theta\right) \mathcal{H}_x\\
\mathcal{H}_x^0
\end{array}\right]v=\mathbbold{0}_{Tm+n}
\end{equation}
This gives 
\begin{equation}\label{eq:fullC_null}
\begin{split}
&\mathcal{H}_u^k v=\hat{\theta}\mathcal{H}_x^k v \text{ for  } k=0,\cdots,T-1\\
&\mathcal{H}_x^0v =\mathbbold{0}_{n}  
\end{split}    
\end{equation} 


% When $C$ is full-rank square matrix, we have  $y(k+1)=C\bm{x}(k+1)=C(A \bm{x}(k)+B u(k))=CA C^{-1}y(k)+CB u(k)$. Hence,
From $\bm{x}(k+1)=A \bm{x}(k)+B u(k)$, we have
\begin{equation}
    \mathcal{H}_x^{k+1}=A \mathcal{H}_x^{k}+B \mathcal{H}_u^{k}
\end{equation}


Pluging in~\eqref{eq:fullC_null} yields 
$\mathcal{H}_x^k v =\mathbbold{0}_{n}$ and $\mathcal{H}_u^k v =\mathbbold{0}_{m}$ for $ k=0,\cdots,T-1$. Hence, $\mathcal{H}v = \mathbbold{0}_{Tm+Tn} $. Namely, $v\in\mathcal{N}(\mathcal{H})$.


Note that $H\in\real^{(Tm+Tn) \times (L-T+1)}$. If $\text{rank}(\mathcal{H})=n+Tm$, then the rank of Null space is $\text{rank}(\mathcal{N}(\mathcal{H}))=(L-T+1)-(n+Tm)$.  
Since $\mathcal{N}(G_\theta)$ is  the same as $\mathcal{N}(\mathcal{H})$, then $\text{rank}(\mathcal{N}(G_\theta))=(L-T+1)-(n+Tm)$.  It follows directly that $\text{rank}(\mathcal{H})=(L-T+1)-\text{rank}(\mathcal{N}(G_\theta))=n+Tm$. 


 


% ************
% Split the first $m$ row of the Hankel matrix gives
% \begin{equation}
% G_\theta:=
% \left[\begin{array}{c}
% [\bm{U}_{0, T, L-T+1} ]_{0}-\hat{\theta}[\bm{X}_{0, T, L-T+1} ]_{0}\\
% \hline
% [\bm{U}_{0, T, L-T+1} ]_{1:T-1} -\left(I_{T-1}\otimes\theta\right)[\bm{X}_{0, T, L-T+1} ]_{1:T-1}\\
% \hline
% [\bm{X}_{0, T, L-T+1} ]_{0}
% \end{array}\right]
% \end{equation}
% If $\text{rank}(G_\theta)<n+Tm$, then there exists a nonzero vector $v\in\real^{Tm+n}$ such that $v^\top G_\theta=\mathbbold{0}_{L-T+1}$. We split the vector $v$ such that $v=(v_0, v_1,v_2) $, where $v_0=[v]_{0:m-1}$, $v_1=[v]_{m:Tm-1}$, $v_2=[v]_{Tm:Tm+n-1}$. Then
% \begin{equation}
% \begin{split}
% v^\top G_\theta=& v_0^\top \left([\bm{U}_{0, T, L-T+1} ]_{0}-\hat{\theta}[\bm{X}_{0, T, L-T+1} ]_{0}\right)+v_2^\top \left([\bm{X}_{0, T, L-T+1} ]_{0}\right)  \\
% &\quad+v_1^\top \left([\bm{U}_{0, T, L-T+1} ]_{1:T-1} -\left(I_{T-1}\otimes\theta\right)[\bm{X}_{0, T, L-T+1} ]_{1:T-1}\right)\\
% =& \left[\begin{array}{cc}
% v_0^\top&v_1^\top
% \end{array}\right]\bm{U}_{0, T, L-T+1} 
% +
% \left(-v_0^\top\hat{\theta}+v_2^\top\right)[\bm{X}_{0, T, L-T+1} ]_{0}\\
% &\quad-v_1^\top \left(I_{T-1}\otimes\theta\right)[\bm{X}_{0, T, L-T+1} ]_{1:T-1}
% \\
% =& \left[\begin{array}{ccc}
% v_0^\top&v_1^\top&-v_0^\top\hat{\theta}+v_2^\top
% \end{array}\right]
% \left[\begin{array}{c}
% \bm{U}_{0, T, L-T+1} \\
% \left [\bm{X}_{0, T, L-T+1} \right ]_{0}
% \end{array}\right]\\
% &\quad-v_1^\top \left(I_{T-1}\otimes\theta\right)M_y
% \left[\begin{array}{c}
% \bm{U}_{0, T, L-T+1} \\
% \left [\bm{X}_{0, T, L-T+1} \right ]_{0}
% \end{array}\right]
% \end{split}
% \end{equation}
\end{proof}


% From~\eqref{eq:Hankel_u_\bm{x}(k)ransition}, the null space $\mathcal{N}(\mathcal{H})$ of the Hankel matrix  is $(L-T+1)-(n+Tm)$.
% If $\bm{x}(t)$ is fully observable( or the length of $\bm{x}(t)$ is the same as $\bm{x}(t)$), then  the rank of null space $\mathcal{N}(G_\theta)$ is also $(L-T+1)-(n+Tm)$. 


If $\text{rank}(G_\theta)=n+Tm$, then there exist at least one solution such that~\eqref{eq:traj_g0} holds. We pick the  minimum-norm solution of~\eqref{eq:traj_g0} given by


\begin{equation}
    g=G_\theta^\top\left(G_\theta G_\theta^\top\right)^{-1}\left[\begin{array}{c}
\bm{w}(0) \\
\vdots\\
\bm{w}(T-1)\\
\bm{x}(0)
\end{array}\right].
\end{equation}

% \wc{I feel that we may not need to involve the case when historic trajectory is not enough. It increases lots of hyper-parameters that is not easy to elaborate clearly.}
%  During the period of data collection, the length of historic trajectory may not be long enough and thus  $\text{rank}(G_\theta)<n+Tm$. In this case, we do not have to wait until the rank condition holds.  We generate trajectory by minimizing the reconstruction error $\min_g ||G_\theta g-[\bm{w}(0),\cdots,\bm{w}(T-1),\bm{x}(0)]^\top||_2^2$, which yields the closed-form solution
%  \begin{equation}
%     g=\left(G_\theta^\top G_\theta \right)^{-1}G_\theta^\top\left[\begin{array}{c}
% \bm{w}(0) \\
% \vdots\\
% \bm{w}(T-1)\\
% \bm{x}(0)
% \end{array}\right]
% \end{equation}


The proposed trajectory generation algorithm is illustrated as follows

\begin{algorithm}
 \caption{Policy Gradient with trajectory generation when the state is observable }
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Require: }}
 \renewcommand{\algorithmicensure}{\textbf{Data collection:}}
 \REQUIRE  The length $T$ of trajectory to be generated, the dimension of state $n$, the dimension of action $m$, the learning rate $\alpha$
 \ENSURE Collect historic measurement of the system and stack each $T$-length input-output trajectory  as Hankel matrix $\mathcal{H}$ shown in~\eqref{eq:Hankel_u_x} until  $\text{rank}(\mathcal{H})=n+Tm$ \\
  \renewcommand{\algorithmicensure}{\textbf{Policy Gradient with Data generation:}}
 \ENSURE 
%  Generate a batch of $Q$ trajectories of the length $T$ subject to the control law $u(t)=\theta \bm{x}(t)+\bm{w}(t)$, $\bm{w}(t)\sim \mathcal{D}$.  \\
 \textit{Initialisation} :Initial weights $\theta$ for control network
 \FOR {$episode = 1$ to $I$}
 \STATE Plug in $\theta$ to compute $G_\theta=\begin{bmatrix}
\mathcal{H}_u-\left(I_{T}\otimes\theta\right) \mathcal{H}_x\\
\mathcal{H}_x^0
\end{bmatrix}$
 \FOR {$i = 1$ to $Q$}
 \STATE Uniformly sample $x^i(0)$ from historic measurement of the system. Sample $\left\{w^i(0),\cdots,w^i(T-1)\right\}$ from the distribution $\mathcal{D}$.
 \STATE Compute the  coefficient $g_i=G_\theta^\top\left(G_\theta G_\theta^\top\right)^{-1}\left[
w^i(0)^\top 
\cdots
w^i(T-1)^\top
x^i(0)^\top
\right]^\top$
\STATE Generate the $i$-th trajectory    $\tau_i:=\left[
\Tilde{\bm{u}}^i(0)^\top 
\cdots
\Tilde{\bm{u}}^i(T-1)^\top
\Tilde{\bm{x}}^i(0)^\top 
\cdots
\Tilde{\bm{x}}^i(T-1)^\top
\right]^\top=\mathcal{H}g_i$
 \ENDFOR
 \STATE Compute the gradient $ \nabla J(\theta) =  \frac{1}{Q}\sum_{i=1}^{Q} c(\tau_i)\sum_{t=1}^{T} \nabla_{\theta}\log\pi_{\theta} (\Tilde{\bm{u}}^i(t)|\Tilde{\bm{x}}^i(t)) $
  \STATE  Update weights in the neural network by gradient descent:
  $\theta \leftarrow \theta-\alpha \nabla J(\theta) $
  \ENDFOR
 \end{algorithmic} 
 \end{algorithm}





==> intro.tex <==
We study the control of networked physical systems, where a large number of individual subsystems are connected to each other and operate in tandem. Such networked systems are present in numerous applications, and understanding their behaviors has been an active line of research~\cite{arcak2016networks,coogan2014dissipativity,simpson2018equilibrium}.
Currently, much of the effort have focused on characterizing properties of the subsystems and their interconnections to certify system stability. At the same time, the performance of these systems, that is, their ability to achieve certain objectives, is also of critical importance. The existing approaches, however, do not offer a framework to optimize system performance. 

In this paper, we develop structured neural network-based controllers that not only guarantee stability, but also establishes a framework for performance optimization. In particular, we consider networked systems where the output of the subsystems need to reach an agreement at the steady state~\cite{burger2014duality,dorfler2014synchronization}. For example, vehicles in a platoon need to reach the same velocity~\cite{coogan2014dissipativity}  and generators in a power grid need to reach the same speed~\cite{cui2022tps}. This steady state should also be reached as quickly as possible, making transient performance of the system important. At the steady state, we want to select the control that achieves output agreement with the lowest possible cost.
% since there are often many set points at the individual systems that lead to the same output value at the steady state, we want to find one that also optimize the cost.
% the transient process before reaching the steady state should 

% We study the control  of safety-critical  networked systems, where  individual physical systems are interconnected to realize cooperative target, including output agreement and performance optimization~\cite{arcak2016networks, burger2014duality, cui2021reinforcement, coogan2014dissipativity}. Such networked system should be stable under control, meaning that the system need to settle down to an acceptable steady state after a disturbance happens~\cite{arcak2016networks, coogan2014dissipativity}. Transient process refers to the period before reaching the steady-state, and the goal of controller design for transient stage is to reach steady state quicker with lower control effort. In addition, we aim to regulate the points where the control actions settles down, such that the required output agreement is attained 
% with the minimum cost~\cite{burger2014duality, Zhao2015acc,jiang2022stable}.
% For example, power systems consist of synchronous generators that are interconnected by the transmission lines. These generators are required to reach the agreement of synchronous with the same speed (60 Hz in North America).  Since there are many ways to set generator power outputs  to achieve this, we would like the output of generators to settle down to the configuration where  the total generation cost is minimized~\cite{Zhao2015acc, jiang2022stable}. 



% Each node only observe the local information and sometimes can communicate with limited neighbours, thus  static local control law and distributed algorithms are required to realize optimization targets.  These controller should still guarantee  stability and output agreement. Moreover, we want to optimize the controllers to realize better performance, which typically include reducing smaller control effort and smaller state deviation from their targeted value.

For the system without real-time computation capability, linear Proportional-Integral (PI)  controllers are almost always used in practice to achieve the above goals~\cite{Zhao2015acc, andreasson2014distributed,  weitenberg2018exponential, golnaraghi2017automatic}. 
A proportional term provides instant feedback to improve the transient performance and an integral term drives the system outputs to the desired value at the steady state~\cite{Zhao2015acc, andreasson2014distributed}. 
% Importantly, linear PI controllers have provable stability guarantees for a large range of systems.
If communication is available, previous works~\cite{Zhao2015acc, andreasson2014distributed,  weitenberg2018exponential, golnaraghi2017automatic, SCHIFFER2017auto} also tailor the integral term to realize distributed optimal resource allocation under quadratic costs. A linear parameterization, however, fundamentally restricts the degrees of freedom of a controller and can lead to very suboptimal performances. 
  

% Learning-based approaches have been proposed to parameterize nonlinear controllers as neural networks, which are then trained to optimize performance~\cite{zhang2021multi, qu2020scalable, wang2021multi,chu2019multi}. However, providing provable guarantees on stability and steady-state optimality has been challenging. In particular, it is nontrivial to certify stability for \textit{all} the possible initial states in a compact set. Recent works showed that monotonic controllers provably stabilize the system~\cite{cui2022tps,shi2021stability}, but they rely on  tailor-made Lyapunov functions and are limited to specific applications.
% %~\cite{huang2019adaptive,chen2021reinforcement}

In the last decade, learning based approaches become popular for nonlinear controller optimization over a host of objective functions~\cite{zhang2021multi, qu2020scalable, wang2021multi,chu2019multi}. The nonlinear control law is normally represented through neural networks, which can then be optimized through learning algorithms.  Many empirical works show that learning based approaches improve the performance by  at least 10\%-50\%  compared with conventional linear approaches for problems on robotics \cite{he2020reinforcement}, traffic systems~\cite{yuan2022reinforcement}, power systems~\cite{wang2021multi, shi2021stability, cui2022tps, cui2021lyapunov}, etc. However, providing provable guarantees on stability and steady-state optimality has been challenging. 

In particular, it is nontrivial to certify stability for \textit{all} the possible initial states in a compact set.  Most works require a linear system model, and sometimes also linear controller, such as LQR problems and its variants~\cite{fazel2018global, lisafe}. Decentralized and distributed neural network-based controller design are proposed to reduce the dependency on communications and global state observations~\cite{li2021distributed, mukherjee2020distributed}. 
The stability for nonlinear system model is more difficult. Many works add soft penalty on the violation of stability conditions in the cost function, but it cannot guarantee stability for all the possible initial states~\cite{chang2019neural}. 
Our previous works in~\cite{furieri2022distributed, cui2022tps,shi2021stability} shows that stabilizing structure can be enforced in the design of neural networks, but  they rely on  tailor-made Lyapunov functions and are limited to specific applications.
%~\cite{huang2019adaptive,chen2021reinforcement}




Moreover, current learning-based approaches generally only optimize transient performance but neglect optimality at the steady-state. Even when training with long time horizons is computationally feasible, it is difficult to quantify how long is enough to cover the steady state. On the other hand, linear PI controllers can achieve stability and steady-state optimality for a large range of systems. This work addresses the following open question:
 \textit{Can learning be structured to guarantee stability and steady-state optimality for a generalized class of networked systems?}


Clearly, it is not possible to design a controller for everything and the answer depends on picking the right abstraction of the system. Passivity is a classical notion in control theory to characterize the inherent property of dynamical
systems by how their inputs and outputs correlate~\cite{arcak2016networks}. Many systems have been shown to be equilibrium-independent
passive (EIP)~\cite{burger2014duality,cui2022equilibrium,meissen2017passivity}, which characterize passivity referenced to an arbitrary equilibrium input/output pair. This abstraction allows us to design generalized controllers for networked systems without considering their detailed dynamics. 
% This provides benefits for  generalized controller design, where the network-level study is based on passivity properties as abstractions of their detailed dynamical models.

\textbf{Contributions.} This paper focuses on controller design for networked systems where the node dynamics are EIP. We propose a structured neural-PI controller that has provable guarantees on stability and achieves steady-state optimal resource allocation. The key structure we use are monotonically increasing functions, and they are parameterized by what we call \emph{monotone neural networks}. This way, transient performances are optimized by training neural networks, while stability and steady-state optimality are guaranteed by design. Experiments on traffic and power system control demonstrate that the proposed approach can reduce the transient cost by at least 30\% compared to the best linear controllers and ensure the optimal steady state cost.  Unstructured neural networks, on ther other hand, lead to unstable behaviors. We summarize contributions as follows.
\begin{enumerate}[noitemsep,nolistsep,leftmargin=*, label=\arabic*)]
    \item We construct a framework of neural network-based controller design that optimizes both transient and steady-state behavior of networked systems. We adopt a modular approach of stability analysis based on equilibrium-independent passivity, making the framework scalable to large systems and also robust to topology and parameter variations.
    \item For networked systems without communication, we propose a neural-PI control law that can be implemented fully decentralizedly with only local information. In Theorem~\ref{thm: output_level_stable}, we prove that the controller design guarantees asymptotic stability and output agreement at the target value. In Theorem~\ref{thm:stack_relu}, we explicitly characterize the structural conditions of monotone neural networks and prove their universal approximation capability of monotonic functions.
    %the controller design and engineer neural networks to satisfy them implicitly. 
    \item If a communication network is available, we propose a neural-PI control law where neighbouring nodes can exchange information of their marginal costs. In Theorem~\ref{thm:equilibrium_cost}, we prove that this design guarantees both stability criteria and steady-state optimal resource allocation for a range of functions that includes, but is not restricted to, quadratic cost functions. 
\end{enumerate}




    %  All of the controllers are structured with monotonic increasing functions,
% allowing us to engineer neural networks and thus achieve steady-state performance guarantee by design. This provide a tractable approach optimize transient performances by learning while.
    % For the networks with communication, we propose structured controller design such that the steady-state optimal resource allocation can also be guaranteed with zero tracking error. This is realized by local updates with limited information exchange with neighbours, which indicates that the setpoints directly settle down to the optimal resource allocation solution distributedly without centralized optimization.

